Preference Modeling with Context-Dependent Salient Features

We consider the problem of estimating a ranking on a set of items from noisy pairwise comparisons given item features. We address the fact that pairwise comparison data often reflects irrational choice, e.g. intransitivity. Our key observation is that two items compared in isolation from other items may be compared based on only a salient subset of features. Formalizing this framework, we propose the salient feature preference model and prove a finite sample complexity result for learning the parameters of our model and the underlying ranking with maximum likelihood estimation. We also provide empirical results that support our theoretical bounds and illustrate how our model explains systematic intransitivity. Finally we demonstrate strong performance of maximum likelihood estimation of our model on both synthetic data and two real data sets: the UT Zappos50K data set and comparison data about the compactness of legislative districts in the US.

==> latexmkrc.tex <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> latexmkrc_2.tex <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> main/conclusion.tex <==
%Focusing on the problem of learning a ranking from pairwise comparison data with irrational choice behaviors, we formulated a random utility model that takes context of the comparison into account when making a comparison judgment. Our model projects the features and judgment vector into a subspace defined by salient features in order to make the comparison. We derived the associated MLE for this model, proved a necessary and sufficient condition for its identifiability, and proved sample complexity bounds for the MLE. Our synthetic experiments illustrated that our model results in comparisons that are intransitive and don't always agree with the overall true rank, something that is often observed in real data. On real data, our model is able to significantly outperform BTL for predicting held-out comparison results. Going forward, we are very interested in understanding a way to identify what selection function $\tau$ people are using for a particular dataset -- whether that means identifying the threshold or developing a nonparametric approach to estimating this model. We are also interested in developing techniques to identify the implicit salient features that are being used for comparison, as opposed to assuming the pre-computed features are the ones being used for comparison.  

We focused on the problem of learning a ranking from pairwise comparison data with irrational choice behaviors, and we formulated the salient feature preference model where one uses projections onto salient coordinates in order to perform comparisons. We proved sample complexity results for MLE on this model and demonstrated the efficacy of our model on both synthetic and real data. Going forward, we would like to develop techniques to learn both the selection function $\tau$ and feature embeddings simultaneously. Finally, it will be useful to consider how to incorporate context into models more sophisticated than BTL, and also consider contextual effects in other tasks that use human judgements such as ordinal embedding \cite{terada2014local}.

% We remark that our model of feature dependent $k$-wise comparisons can be extended to any model that uses comparison judgements such as triplets. And can be extended models that model individual users. Although this model is presented as a modification of the Placket-Luce model, the idea that the features used for ak-wise comparison are dependent on the pairs being compared can be extended to99other models such as ranking SVM.



==> main/district.tex <==
\paragraph{District Compactness}
\cite{districtCompactness} collected preference data to understand human perception of compactness of legislative districts in the United States. % in order to produce a ranking of districts with respect to compactness. 
Their data include both pairwise comparisons and $k$-wise ranking data for $k > 2$ as well as 27 continuous features for each district, including geometric features and compactness metrics. Although difficult to define precisely, the United States law suggests compactness is universally understood \cite{districtCompactness}. In fact, the authors provide evidence that most people agree on a universal ranking, but they found the pairwise comparison data was extremely noisy. They hypothesize that pairwise comparisons may not directly capture the full ranking, since all features may not be used when comparing two districts in isolation from the other districts. Hence, this problem is applicable to our salient feature preference model and its motivation.

\begin{table*}
  \caption{Average Kendall tau correlation over individual rankings on test sets for district compactness. The number in parenthesis is the standard deviation.}
  \label{table:districtResults}
  \centering
  \begin{tabular}{llllllll}
    \toprule
    \cmidrule(r){1-2}
Model:             & \texttt{Shiny1}    & \texttt{Shiny2}    & \texttt{UG1-j1} & \texttt{UG1-j2} & \texttt{UG1-j3} & \texttt{UG1-j4} & \texttt{UG1-j5} \\
    \midrule
Salient features   & \textbf{0.14} (.26) & \textbf{0.26} (.2) & \textbf{0.48} (.21) & \textbf{0.41} (.09) & \textbf{0.6} (.1) & 0.14 (.14) & \textbf{0.42} (.09)    \\ 
FBTL  & 0.09 (.22) & 0.18 (.17) & 0.2 (.12) & 0.26 (.07) & 0.45 (.15) & 0.2 (.13) & 0.06 (.14)    \\ 
Ranking SVM  & 0.09 (.22) & 0.18 (.17) & 0.22 (.12) & 0.26 (.07) & 0.45 (.15) & 0.2 (.13) & 0.06 (.14) \\
% RankNet  & \textbf{0.16} (.28)& \textbf{0.31} (.22)& 0.42 (.06)& \textbf{0.46} (.08)& 0.53 (.11)& 0.05 (.06)& 0.17 (.03) \\
RankNet  & 0.12 (.24)& 0.24 (.18)& 0.28 (.14)& 0.37 (.08)& 0.53 (.11)& \textbf{0.28} (.08)& 0.15 (.15) \\ 
    \bottomrule
  \end{tabular}
\end{table*}

 \begin{table*}
  \centering
  \caption{Average pairwise prediction accuracy over 10 train/validation/test splits on the test sets by attribute for \texttt{UT Zappos50k}. $C$ stands for coarse and $F$ stands for fine grained. The number in parenthesis is the standard deviation.}
  \label{table:zappos}

  \begin{tabular}{lllllllll}
    \toprule
    \cmidrule(r){1-2}
Model:                     & open-$C$ & pointy-$C$ & sporty-$C$ & comfort-$C$ & open-$F$ & pointy-$F$ & sporty-$F$ & comfort-$F$ \\
    \midrule
Salient features     & 0.73 (.02) & 0.78 (.02) & 0.78 (.03) & 0.77 (.03) & 0.6 (.04) & 0.59 (.04) & 0.59 (.03) & 0.56 (.03) \\
FBTL     & 0.73 (.02) & 0.77 (.03) & 0.8 (.03) & 0.78 (.03) & 0.6 (.03) & 0.6 (.03) & 0.59 (.03) & 0.58 (.05) \\
Ranking SVM      & 0.74 (.02) & 0.78 (.03) & 0.79 (.03) & 0.78 (.03)  & 0.6 (.03) & 0.6 (.04) & 0.6 (.04) & 0.58 (.03)\\
RankNet  & 0.73 (.01) & 0.79 (.01) & 0.78 (.03) & 0.8 (.02) & 0.61 (.02) & 0.59 (.02) & 0.59 (.04) & 0.59 (.05) \\ 

    \bottomrule
  \end{tabular}
\end{table*}

The goal as set forth by \cite{districtCompactness} is to learn a ranking of districts. We train on 5,150 pairwise comparisons collected from 94 unique pairs of districts to learn $\hat{w}$, an estimate of the judgment vector $w^*$, then estimate a ranking by sorting the districts by $\langle \hat{w}, U_i\rangle$. The $k$-wise ranking data sets are used for validation and testing.  Since there is no ground truth for the universal ranking, we measure how close the estimated ranking is to each individual ranking. %Furthermore, in this scenario, we care about how accurate the estimated ranking is at any position in the ranking, not just how well it estimates the top items. 
In this scenario, we care about the accuracy of the full ranking, and so we consider Kendall tau correlation.
Given a $k$-wise comparison data set, Table \ref{table:districtResults} shows the average Kendall tau correlation between the estimated ranking and each individual ranking where the number in parenthesis is the standard deviation. The standard deviation on \texttt{shiny1} and \texttt{shiny2} is relatively high because the Kendall tau correlation between pairs of rankings in these data sets has high variability, shown in Figure \ref{fig:intercoder} in the Supplement.

The MLE of the salient feature preference model under the top-$t$ selection function outperforms both the MLE of FBTL and Ranking SVM by a significant amount on 6 out 7 test sets, suggesting that pairwise comparison decisions may be better modeled by incorporating context. The MLE of the salient feature preference model, which is linear, is competitive with RankNet, which models pairwise comparisons as in Equation \eqref{eq:BTL} except where the utility of each item uses a function  $f$ defined by a neural network, i.e. $u_i = f(U_i)$.

The salient feature preference model may be outperforming FBTL and Ranking SVM since this data exhibits significant violations of rational choice. First, on the training set of pairwise comparisons, there are 48 triplets of districts $(i,j,k)$ where both (1) all three distinct pairwise comparisons were collected and (2) $P_{ij} > .5$ and $P_{jk} > .5$. Seventeen violate strong transitivity, 3 violate moderate transitivity, but none violate weak transitivity. 
%Furthermore, 13 violate strong stochastic transitivity by at least $5\%$, meaning if $P_{ij} \geq .5$ and $P_{jk} \geq .5$, then $P_{ik} \leq \max\{P_{ij}, P_{jk}\} - .05$, and 1 violates moderate stochastic transitivity by $5\%$. 
Second, given a set of $k$-wise ranking data, let $\hat{P}_{ij}$ be the proportion of rankings in which item $i$ is ranked higher than item $j$.
%times item $i$ is ranked higher than item $j$ over all the $k$-wise rankings. 
There are 20 pairs of districts that appear in both the $k$-wise ranking data and
% as well as
the pairwise comparison training data. Four of these pairs of items $i,j$ have the property that $(.5 - P_{ij})(.5 - \hat{P}_{ij})<0$, meaning item $i$ is typically ranked higher than item $j$ in the ranking data, but $j$ typically beats $i$ in the pairwise comparisons.



==> main/experiments.tex <==
\label{sec:experiments}
See Sections \ref{appendix:algorithmImplementation}, \ref{appendix:district_experiments}, and \ref{appendix:zappos} of the Supplement for additional details about the algorithm implementation, data, preprocessing, hyperparameter selection, and training and validation error for both synthetic and real data experiments. 
%Recall, the FBTL model is the BTL model with features, i.e. Equation \eqref{eq:BTL} where $u_i = \langle U_i, w^* \rangle$ for $i \in [n]$. 
% Throughout this section, the BTL model refers to Equation \eqref{eq:thresholdBTL} with the constant selection function $\tau(i,j) = [d]$ for $i,j \in [n]$.
% the BTL model where the utility of item $i$ is given by $\langle U_i, w^* \rangle$. 
% We refer to the BTL model where the utility of an item is arbitrary given by Equation \eqref{eq:BTL} as the BTL without features model. We refer to either of these models as the BTL model when it is not important to differentiate them.
\subsection{Synthetic Data}
\subfile{synthetic_experiments}
\label{sec:syntheticExperiments}

\subsection{Real Data}
\label{sec:realDataExp}
For the following experiments, we use the top-$t$ selection function for the salient feature preference model, where $t$ is treated as a hyperparameter and tuned on a validation set. 
We compare to FBTL, RankNet \cite{burges2005learning} with one hidden layer, and Ranking SVM  \cite{joachims2002optimizing}. We append an $\ell_2$ penalty to $\mathcal{L}_m$ for the salient feature preference model and the FBTL model, that is, for regularization parameter $\mu$, we solve $\min_{w \in \mathbb{R}^d} \mathcal{L}_{m}(w) + \mu\|w\|^2_2.$ For RankNet, we add to the objective function an $\ell_2$ penalty on the weights. As explained in more detail in subsections \ref{appendix:districtHyperparameters} and \ref{appendix:zapposHyperparameters} in the Supplement, the hyperparameters for the salient feature preference model are $t$ for the top-$t$ selection function and $\mu$, the hyperparameter for FBTL is $\mu$, the hyperparameter for Ranking SVM is the coefficient corresponding to the norm of the learned hyperplane, and the hyperparameters for RankNet are the number of nodes in the single hidden layer and the coefficient for the $\ell_2$ regularization of the weights.

\subfile{district.tex}
\subfile{zappos.tex}

==> main/intro.tex <==
The problem of estimating a ranking is ubiquitous and has applications in a wide variety of areas such as recommender systems, review of scientific articles or proposals, search results, sports tournaments, and understanding human perception. Collecting full rankings of $n$ items from human users is infeasible if the number of items $n$ is large. Therefore, $k$-wise comparisons, $k<n$, are typically collected and aggregated instead. % since $k! \ll n!$ for small $k$. The idea is that it is relatively easy to rank $k$ items with the additional cost of deciding which ${n \choose k}$ different $k$-wise comparisons to collect. For instance, if $k=2$, these $2$-wise comparisons are known as pairwise comparisons. 
Pairwise comparisons ($k=2$) are popular since it is believed that humans can easily and quickly answer these types of comparisons. However, it has been observed that data from $k$-wise comparisons for small $k$ often exhibit what looks like irrational choice, such as systematic intransitivity among comparisons. Common models address this issue with modeling noise, ignoring its systematic nature. We observe, as others have before us \cite{seshadri2019discovering, rosenfeld2019predicting, DBLP:journals/corr/abs-1901-10860, kleinberg2017comparison, benson2016relevance, chen2016predicting, Chen:2016:MIM:2835776.2835787}, that these systematic irrational behaviors can likely be better modeled as \emph{rational behaviors made in context}, meaning that the particular $k$ items used in a $k$-wise comparison will affect the comparison outcome.

Consider the most common model for learning a single ranking from pairwise comparisons, the Bradley-Terry-Luce (BTL) model. In this model, there exists a judgment vector $w^* \in \R^d$ that indicates the favorability of each of the $d$ features of an item (e.g. for shoes: cost, width, material quality, etc), and each item has an embedding $U_i \in \R^d$, $i=1,\dots,n$, indicating the value of each feature for that given item. Subsequently, the outcome of a comparison is made with probability related to the inner product $\langle U_i, w^* \rangle$; the larger this inner product, the more likely item $i$ will be ranked above other items to which it is compared. A key implicit assumption is that the features used to rank all $n$ items are the same features used to rank just $k$ items in the absence of the other $n-k$ items. %In other words, it is assumed that given $k$ items, a sampled $k$-wise comparison will be very similar to the ordering of these $k$ items in the underlying ranking $\sigma^*$.
However, %this assumption may be violated. In particular, when each item has many different features,  
%in certain scenarios, 
we argue that the context of that particular pairwise comparison is also relevant; it is likely that %when the items are ranked altogether at once, every feature is taken into account, but 
when a pairwise comparison is collected, if there are a small number of features that ``stand out,'' a person will use only these features and ignore the rest when he or she makes a comparison judgment. Otherwise, if there are no salient features between a pair of items, a person will take all features into consideration. This theory has been hypothesized by the social science community to explain violations of rational choice \cite{tversky1972elimination, tversky1993context, rieskamp2006extending, brown2009enquiry, shepard1964attention, torgerson1965multidimensional, tversky1977features, bordalo2013salience}. % \begin{quote}
% When people compare multiattribute options, the similarity of values along one attribute enhances differences on other attributes. These comparability effects are easily linked to cognitive processing. When evaluating options, people pay more attention to attributes that differ. \cite{rieskamp2006extending}. \todo{can remove for space}
% \end{quote}%For example, this issue has been highlighted and explored empirically in \cite{districtCompactness}, where the authors initially attempted to use pairwise comparisons to understand human perception of legislative district compactness but then decided to abandon pairwise comparisons for $k$-wise comparisons where $k \in \{20, 100\}$. 
% Furthermore, \todo{CITE ML textbook} also speaks about this issue with no resolution.
For example, \cite{districtCompactness} collected preference data to understand human perception of the compactness of legislative districts. They hypothesized that the features respondents use in a pairwise comparison task to judge district compactness vary from pair to pair, which explains why their data are more reliable for larger $k$. To illustrate this point, we highlight a concrete example from their experiments. Given two images of districts, they asked respondents to pick which district is more compact. When comparing district $A$ with district $B$ or district $C$ in Figure \ref{fig:districts}, one of the most salient features is the degree of nonconvexity. However, when comparing district $B$ and district $C$, the degree of nonconvexity is no longer a salient feature. These districts look similar on many dimensions, forcing a person to really think and consider all the features before making a judgment.
%such as the ``thin" region in the middle of district $C$ and its long and thin shape. \todo{there are two ways to go: (1) argue that some feature stands out between B and C. Does something stand out to you? or (2) say that they look the same, so all features will be used, in which case we need to add this reasoning to this paragraph.} 
Let $P_{ij}$ be the empirical probability that district $i$ beats district $j$ with respect to compactness. Then, from the experiments of \cite{districtCompactness}, we have $P_{AB} = 100\%$, $P_{BC} = 67\%$, and $P_{AC} = 70\%$. These three districts violate strong stochastic transitivity, the requirement that if $P_{AB} \geq 50\%$ and $P_{BC} \geq 50\%$, then $P_{AC} \geq \max\{P_{AB},P_{BC}\}$.

\begin{figure}[!htb]
\minipage{0.15\textwidth}
\centering
District $A$
  \includegraphics[width=\linewidth]{main/figs/1_U_018_2010.jpg}
%   \caption*{}\label{fig:districtA}
\endminipage\hspace{\fill}
\minipage{0.15\textwidth}
\centering
District $B$
  \includegraphics[width=\linewidth]{main/figs/48_L_050_2010.jpg}
%   \caption*{District $B$}\label{fig:districtB}
\endminipage\hspace{\fill}
\minipage{0.15\textwidth}%
\centering
District $C$
  \includegraphics[width=\linewidth]{main/figs/37_L_075_2010.jpg}
%   \caption*{District $C$}\label{fig:districtC}
\endminipage
\caption{Three districts used in pairwise comparison tasks in \cite{districtCompactness}}
\label{fig:districts}
\end{figure}


We propose a novel probabilistic model called the \textit{salient feature preference model} for pairwise comparisons such that the features used to compare two items are dependent on the context in which two items are being compared. The salient feature preference model is a variation of the standard Bradley-Terry-Luce model. At a high level, given a pair of items in $\R^d$, we posit that humans perform the pairwise comparison in a coordinate subspace of $\R^d$. The particular subspace depends on the salience of each feature of the pairs being compared. Crucially, if any human were able to rank all the items at once, he or she would compare the items in the ambient space without projection onto a smaller subspace. This single ranking in the ambient space %incorporating all the features 
is the ranking that we would like to estimate. Our contributions are threefold. First, we precisely formulate this model and derive the associated maximum likelihood estimator (MLE) where the log-likelihood is convex. Our model can result in intransitive preferences, despite the fact that comparisons are based off a single universal ranking. In addition, our model generalizes to unseen items and unseen pairs. Second, we then prove a necessary and sufficient identifiability condition for our model and finite sample complexity bounds for the MLE. %To the best of our knowledge, ours is the first sample complexity result for learning a ranking on a set of items where the observed pairwise preferences violate transitivity. 
Our result specializes to the sample complexity of the MLE for the BTL model with features, which to the best of our knowledge has not been provided in the literature. Third, we provide synthetic experiments that support our theoretical results and also illustrate scenarios where our salient feature preference model results in systematic intransitives. We also demonstrate the efficacy of our model and maximum likelihood estimation on real preference data about legislative district compactness and the \texttt{UT Zappos50K} data set.

% Our contributions are
% \begin{itemize}
%     \item We propose a novel probabilistic and parametric pairwise preference model that takes into account the context of each pairwise comparison in order to model violations of rational choice better.
%     \item We prove a finite sample complexity result on learning the parameters of our model.
%     \item We consider particular choices of context to better understand our sample complexity results.
%     \item We provide experiment results that demonstrate the efficacy of our model on real data as well as show how violations of rational choice affect the sample complexity for the worse.
% \end{itemize}

% Under the salient feature preference model, we propose using maximum likelihood estimation in order to learn the underlying ranking on the items \todo{is this too vague?}. Theoretically, we prove sample complexity bounds and show how our model interpolates between projection on a small subspace for small $k$ to no projection for large $k$ in which case our salient feature preference model becomes the standard Placket-Luce model or Bradley-Terry-Luce model when $k=2$. We illustrate our theory on synthetic data and also show the efficacy of our model and algorithm on a real world example: paired comparison data on human perception of legislative district compactness.

%\subsection{Contribution} The main contribution of this work is formulating a random utility model for discrete choice on a set of items with an underlying ranking such that the observed $k$-wise comparisons can systematically disagree with the underlying ranking. \todo{This first sentence needs to be changed. I don't like it.} Theoretically, we prove sample complexity bounds for the maximum likelihood estimator of our model. We provide synthetic experiments for our theoretical results and also demonstrate scenarios where the salient feature preference model results in systematic intransitives. We also demonstrate the efficacy of our model and maximum likelihood estimation on real preference data collected.

%and also theoretically justify how our preference salient feature preference model interpolates between the standard Placket-Luce discrete choice model when $k$ is large meaning all features are used when ranking the $k$ items versus using only a small number of features when ranking the $k$ items when $k$ is relatively small

\subsection{Related Work}
\paragraph{The Bradley-Terry-Luce Model}
One popular probabilistic model for pairwise comparisons is the Bradley-Terry-Luce (BTL) model \cite{bradley1952rank, luce2012individual}. In this model, there are $n$ items each with an unknown utility $u_i$ for $i \in [n]$, and the items are ranked by sorting the utilities. The BTL model defines
\begin{align}
\label{eq:BTL}
    \mathbb{P}(\text{item } i \text{ beats item } j) = \frac{e^{u_i}}{e^{u_i}+e^{u_j}}.
\end{align}

Although the BTL model makes strong parametric assumptions, it has been analyzed extensively by both the machine learning and social science community and has been applied in practice. For instance, the World Chess Federation has used a variation of the BTL model in the past for ranking chess players \cite{menke2008bradley}. The sample complexity of learning the utilities or the ranking of the items with maximum likelihood estimation (MLE) has been studied recently in \cite{pmlr-v32-rajkumar14, rankCentrality}. Moreover, there is a recent line of work that analyzes the sample complexity of learning the utilities with MLE and other algorithms under several variations of the BTL model, including when the items have features that may or may not be known \cite{NIPS2018_7746, oh2015collaboratively, lu2015individualized, park2015preference, fbtl, niranjan2017inductive}. Our model is also a variation of the BTL model where the utility of each item is dependent on the items it is being compared to.
%There is a recent line of work that replaces the strong parametric assumptions of BTL with less restrictive assumptions on the pairwise preference matrix $P$ where $P_{ij} = \mathbb{P}(\text{item } i \text{ beats item } j)$ 
%The goals in these works are estimating $P$ or learning a ranking from $P$ by ranking the items by $u_i = \sum_{j=1}^n P_{ij}$ for $i \in [n]$ 
%\cite{falahatgar2018limits, pmlr-v32-rajkumar14, DBLP:journals/corr/ShahW15, rajkumar2016can, Agarwal:2016:RCM:3061053.3061214,shah2017stochastically, Rajkumar:2015:RSP:3045118.3045190}. %However, most of these works assume that $P$ reflects transitive choices although intransitivity is often observed in real data. In our work we demonstrate how intransitivies arise under our model with a reasonable generative model for the items' features implying that transitivity may be a strong and unnecessary assumption in certain real applications.
% In addition to transitivity, seemingly irrational choices may violate \textit{independence from irrelevant alternatives} (IIA), which is another property that preferences from a BTL model must satisfy. One version of IIA says for all quadruples $(i,j,k,\ell)$ if $P_{ik}\geq P_{jk}$, then $P_{i\ell}\geq P_{j\ell}$. At a high level, IIA means that choices between items do not depend on the context in which they are shown. \todo{this sentence feels out of place}

% {\color{orange} When each item $i$ has features $U_i \in \mathbb{R}^d$, a common way to incorporate the features into the utilities is to assume there is a judgment vector $w^* \in \mathbb{R}^d$ so that the utility of item $i$ is $\langle U_i, w^* \rangle$ \cite{rieskamp2006extending}. There is a recent line of work that analyzes the sample complexity of learning the utilities with MLE and other algorithms under several variations of the BTL model when the items have features that may or may not be known and when there may be multiple $w^*$ corresponding to different individuals \cite{NIPS2018_7746, oh2015collaboratively, lu2015individualized, park2015preference, f-btl, niranjan2017inductive}. The BTL model is a random utility model for discrete choice, which models choice as a noisy process that depends on the utilities of items \cite{thurstone1927law}. Our model, which is a modification of the BTL model, is also a random utility model where the utility of an item is dependent on the item being compared to, as opposed to the BTL model where the utility of each item is independent of the pairwise comparison. } \laura{this needs rearranging}
%We seek to estimate $w^*$ in order to estimate a ranking on the items and estimate the pairwise probabilities.

% \paragraph{The pairwise preference matrix}
% The BTL model makes strong parametric assumptions about how pairwise rankings are distributed. There is a recent line of work that replaces these strong parametric assumptions with more general, less restrictive assumptions on the $n \times n$ pairwise preference matrix $P$ where $P_{ij} = \mathbb{P}(\text{item } i \text{ beats item } j)$ with various goals such as estimating $P$ or learning a ranking from $P$ by ranking the items by $\sum_{j=1}^n P_{ij}$ \cite{falahatgar2018limits, pmlr-v32-rajkumar14, DBLP:journals/corr/ShahW15, shah2016stochastically, rajkumar2016can, Agarwal:2016:RCM:3061053.3061214,shah2017stochastically, Rajkumar:2015:RSP:3045118.3045190}. However, most of these works assume $P$ satisfies either weak or strong stochastic transitivity: for any triplets $(i,j,k)$, if $P_{ij} \geq \frac{1}{2}$ and $P_{jk} \geq \frac{1}{2}$, then weak stochastic transitivity implies $P_{ik} \geq \frac{1}{2}$ and strong stochastic transitivity implies $P_{ik} \geq \max\{P_{ij}, P_{jk}\}$. \cite{rieskamp2006extending} %though we remark that in \cite{shah2017stochastically} the implication is that $P_{ik} \geq P_{jk}$. \todo{is it necessary to point out this difference?} 
% The BTL model satisfies strong and hence weak stochastic transitivity.

% In our work we propose a probabilistic model for pairwise comparisons that may violate stochastic transitivity and demonstrate this violation with a reasonable generative model implying that stochastic transitivity is a strong and unnecessary assumption in certain real applications.

\paragraph{Violations of Rational Choice}
The social science community has long recognized and hypothesized about irrational choice \cite{shepard1964attention, torgerson1965multidimensional, tversky1977features, tversky1972elimination, bordalo2013salience}. See \cite{rieskamp2006extending} for an excellent survey of this area including references to social science experiments that demonstrate scenarios where humans make choices that can violate a variety of rational choice axioms such as transitivity.
%
% We base our preference model on theory that in certain scenarios, irrational choice can arise because items are multidimensional:
% \begin{quote}
% A prominent hypothesis for why such intransitivities occur is that people tend to pay more attention to those attributes for which the values differ substantially, deemphasizing attributes that do not as dramatically distinguish the options. When different choices lead people to focus on different attributes, intransitivity may result \cite{brown2009enquiry}.  
% \end{quote}
% \begin{quote}
% When people compare multiattribute options, the similarity of values along one attribute enhances differences on other attributes. These comparability effects are easily linked to cognitive processing. When evaluating options, people pay more attention to attributes that differ. \cite{rieskamp2006extending}. 
% \end{quote}
% \todo{which quote do you like more? or do you want to remove them} 
% \todo{I'm wondering if this paragraph this would actually be more appropriate to talk about AFTER we precisely define our model as a justification? }
%When a person sees a pair of items in isolation from the rest of the items, there may be certain features that ``stand out'' which means other less prominent features may be ignored when making the isolated pairwise comparison: 
%
% Furthermore, we restrict ourselves to scenarios where we believe a ranking on the items exists and take this theory one step further: if all the items are observed at once, all the features will be used when comparing the items. \todo{is this believable/too informal?} The work, which motivated us, in \cite{districtCompactness} is an example of this scenario. They aimed to understand human perception of the compactness of legislative districts through comparison data and posited that pairwise comparisons were unreliable compared to $k$-wise rankings because each district has many features. These authors also provided some evidence of the existence of a ranking in their application that most people agree on even if the pairwise comparison data did not directly reflect this. 
%ragain2016pairwise, kleinberg2017comparison, benson2016relevance, Rajkumar:2015:RSP:3045118.3045190, dehui
There has been recent progress in modeling and providing evidence for violations of rational choice axioms in the machine learning community \cite{seshadri2019discovering, rosenfeld2019predicting, heckel2019active, DBLP:journals/corr/abs-1901-10860, kleinberg2017comparison, shah2017simple, ragain2016pairwise, niranjan2017inductive, benson2016relevance, chen2016predicting, Chen:2016:MIM:2835776.2835787, Rajkumar:2015:RSP:3045118.3045190, dehui, agresti2012categorical}. In contrast to our work, none of these works model preference data that both violates rational choice and admits a universal ranking of the items with the exception of \cite{shah2017simple,heckel2019active}. Assuming there is a true ranking of the items, our model makes a direct connection between pairwise comparison data that violates rational choice and the underlying ranking. Violations of rational choice, including intransitivty, occur in our model because of contextual effects due to which pairs of items are being compared. These contextual effects distort the true ranking, whereas in the work of \cite{shah2017simple,heckel2019active} the intransitive choices define the ranking. Specifically, the items are ranked by sorting the items by the probability that an item beats any other item.

We now focus on the works most similar to ours. The work in \cite{seshadri2019discovering}, which generalizes \cite{chen2016predicting, Chen:2016:MIM:2835776.2835787} from pairwise comparisons to $k$-wise comparisons, considers a model for context dependent comparisons. However, because they do not assume access to features, their model cannot predict choices based on new items, which is a key task for very large modern data sets. In contrast, our model can predict pairwise outcomes and rankings of new items. Both \cite{rosenfeld2019predicting} and \cite{DBLP:journals/corr/abs-1901-10860} assume access to features of items and propose learning contextual utilities with neural networks. In contrast, we propose a linear approach with typically far fewer parameters to estimate. Furthermore, the latter work does not contain any theory, whereas we prove a sample complexity result on estimating the parameters of our model. In all of the aforementioned works in this paragraph, the resulting optimization problems are non-convex with the exception of a special case in \cite{seshadri2019discovering} that requires sampling every pairwise comparison. In contrast, the negative log likelihood of our model is convex. Interestingly, the work in \cite{makhijani2019parametric} shows that for a class of parametric models for pairwise preference probabilities, if intransitives exist, then the negative log likelihood cannot be convex. Our model does not belong to the class of parametric models they consider.


%     The authors in \cite{seshadri2019discovering} consider a general model for context dependent comparisons. For $n$ items, let $\{u_{x,z}\}_{x,z \in [n]}$ be pairwise contextual utilities so that for a subset of items $C \subset [n]$ and item $x \in [n]$, \[\mathbb{P}(x \text{ is chosen from } C) = \frac{\exp(\sum_{z \in C \setminus \{x\}} u_{x,z})}{\sum_{y \in C }
% \exp(\sum_{z \in C \setminus \{y\}} u_{y,z})}.\] This is a variation of the BTL model for picking the best item from a set, where the utility of an item depends on those it is compared to. Their model in general requires $O(n^2)$ parameters, since they learn a number for every pair, and it also does not allow prediction on unseen pairs. 
%  Therefore, they consider a special case where each item is associated with an unknown target vector and an unknown context vector both in  $\mathbb{R}^d$, so that the context dependent utility is a function of these $O(nd)$ parameters only. %of item $x$ is $(\sum_{z \in C \setminus \{x\}} c_z)^T t_x$. This model only requires $O(nd)$ parameters. 
%  When $|C| =2$, this model reduces to the model of \cite{chen2016predicting, Chen:2016:MIM:2835776.2835787}.


% The authors in \cite{chen2016predicting, Chen:2016:MIM:2835776.2835787} model intransitivity by taking into account the context of the pairwise comparison. In particular, as opposed to the BTL model which assumes that each item has a global utility, their \textit{blade-chest model} like ours proposes a variation of BTL that assigns a utility to each item that depends on the other item it is being compared to. More specifically, they assume each item has two unknown feature vectors $a_{\text{blade}}$ and $a_{\text{chest}}$ where one proposed pairwise distribution is \[\mathbb{P}(\text{item } a > \text{ item } b) = \frac{\exp(\langle a_{\text{blade}}, b_{\text{chest}} \rangle)}{\exp(\langle a_{\text{blade}}, b_{\text{chest}} \rangle) + \exp(\langle b_{\text{blade}}, a_{\text{chest}} \rangle)}.\] The authors provide evidence that real data has intransitivities and find that the MLE of their model outperforms the MLE of the BTL model on head-to-head matchups in online video games. %This work does not provide theory and furthermore our salient feature preference model cannot be written as a blade-chest model.

%  In particular,  they assume each item $x$ is associated with an unknown target vector $t_x \in \mathbb{R}^d$ and an unknown context vector $c_x \in \mathbb{R}^d$
% and propose a variation of the BTL model such that the utility of item $x$ when compared among a set of items $C$ is $(\sum_{z \in C \textbackslash \{x\}} c_z)^T t_x$. In other words, 
% \[\mathbb{P}(x \text{ is chosen from } C) = \frac{\exp((\sum_{z \in C \textbackslash \{x\}} c_z)^T t_x)}{\sum_{y \in C } \exp((\sum_{z \in C \textbackslash \{y\}} c_z)^T t_y)}.\]   
% The former model is called a \textit{low rank context dependent random utility model} since it requires only $nd$ parameters versus the latter model that requires $O(n^2d)$ parameters. They provide sample complexity bounds for learning the pairwise contextual utilities with MLE and provide a statistical test for detecting violations of IIA.

% We now focus on two works most similar to ours. The authors in \cite{chen2016predicting, Chen:2016:MIM:2835776.2835787} model intransitivity by taking into account the context of the pairwise comparison. In particular, as opposed to the BTL model which assumes that each item has a global utility, their \textit{blade-chest model} like ours proposes a variation of BTL that assigns a utility to each item that depends on the other item it is being compared to. More specifically, they assume each item has two unknown feature vectors $a_{\text{blade}}$ and $a_{\text{chest}}$ where one proposed pairwise distribution is \[\mathbb{P}(\text{item } a > \text{ item } b) = \frac{\exp(\langle a_{\text{blade}}, b_{\text{chest}} \rangle)}{\exp(\langle a_{\text{blade}}, b_{\text{chest}} \rangle) + \exp(\langle b_{\text{blade}}, a_{\text{chest}} \rangle)}.\] The authors provide evidence that real data has intransitivities and find that the MLE of their model outperforms the MLE of the BTL model on head-to-head matchups in online video games. %This work does not provide theory and furthermore our salient feature preference model cannot be written as a blade-chest model.

% The work in \cite{seshadri2019discovering} is a generalization of the blade-chest model. In particular, they assume each item $x$ is associated with an unknown target vector $t_x \in \mathbb{R}^d$ and an unknown context vector $c_x \in \mathbb{R}^d$ and propose a variation of the BTL model such that the utility of item $x$ when compared among a set of items $C$ is $(\sum_{z \in C \textbackslash \{x\}} c_z)^T t_x$. In other words, 
% \[\mathbb{P}(x \text{ is chosen from } C) = \frac{\exp((\sum_{z \in C \textbackslash \{x\}} c_z)^T t_x)}{\sum_{y \in C } \exp((\sum_{z \in C \textbackslash \{y\}} c_z)^T t_y)}.\] More generally, they consider pairwise contextual utilities $\{u_{x,z}\}_{x,z \in [n]}$ and model \[\mathbb{P}(x \text{ is chosen from } C) = \frac{\exp(\sum_{z \in C \textbackslash \{x\}} u_{x,z})}{\sum_{y \in C } \exp(\sum_{z \in C \textbackslash \{y\}} u_{y,z})}.\]  The former model is called a \textit{low rank context dependent random utility model} since it requires only $nd$ parameters versus the latter model that requires $O(n^2d)$ parameters. They provide sample complexity bounds for learning the pairwise contextual utilities with MLE and provide a statistical test for detecting violations of IIA.

% Our model is a special case of their model with arbitrary pairwise contextual utilities. However, our model is convex, and we only require learning $d$ parameters since we utilize known item features to model the pairwise contextual utilities. In contrast to their model, our model can predict pairwise comparisons and ranking of new items, which is a key task for very large modern datasets. Furthermore, we are able to provide a more complete characterization of identifiability. %Because we make assumptions about how humans make pairwise comparison decisions with respect to the underling ranking of items, we can estimate a ranking of the items, whereas their very general model cannot since they are not necessarily assuming the existence of an underlying ranking. \todo{rewrite this? point out differences between our work and what we contribute }

%In \cite{ragain2016pairwise}, the authors propose a probabilistic model for $k$-wise comparisons which depends on the stationary distribution restricted to the $k$ items of a Markov chain on a directed graph whose nodes correspond to the items. \todo{too vague/confusing?} In general, the resulting model will not satisfy transitivity and again incorporates context information based on which items are being compared. They propose MLE for inference and prediction. The authors in \cite{kleinberg2017comparison} consider a class of choice models that may violate IIA and seek to understand the algorithmic limits of inferring the underlying choice model. The work in \cite{benson2016relevance} provides empirical evidence for violations of IIA and provide an novel algorithm inspired by a model from social choice theory.  \todo{the deatlis of these last 3 references aren't super relevant, so maybe try to consolidate this to a sentence and say people have been working on models/algorithms when IIA/transitivity is violated}

% \paragraph{Organization} The remainder of this paper is organized as follows. In Section \ref{sec:modelFormulation}, we formalize the salient feature preference model and the maximum likelihood algorithm we use to estimate the underlying ranking on items. In Section \ref{sec:theory}, we present sample complexity bounds for the MLE. In Section \ref{sec:experiments}, we present synthetic experiments illustrating our theory as well as applying our model and algorithm to paired comparison data collected about legislative district compactness.
%and theoretically demonstrate the quantitative difference of $k$-wise comparisons for small $k$ versus large $k$ in terms of agreement with the underlying ranking

\paragraph{Notation} For an integer $d>0$, $[d] := \{1, \dots, d\}$. For $x,y \in \mathbb{R}^d$, $\langle x, y \rangle := \sum_{i = 1}^d x_i y_i$. %Given $U \in \mathbb{R}^{d \times n}$, $\lambda_{\text{min}}(U)$ is the smallest eigenvalue of $U$ when $n = d$, $\lambda_{\text{max}}(U)$ is the largest eigenvalue of $U$ when $n = d$, and $\sigma_{\max}(U)$ is the largest singular value of $U$. 
For $x \in \mathbb{R}^d$ and $\Omega \subset [d]$, let $x^{\Omega} \in \mathbb{R}^d$ where $(x^{\Omega})_i = x_i$ if $i \in \Omega$ and 0 otherwise. For $i,j \in [n]$, ``$i >_B j$'' means ``item $i$ beats item $j$.'' Let $\mathcal{P}(X)$ be the power set of a set $X$. Given a set of vectors $S = \{x_i \in \mathbb{R}^d \}_{i = 1}^q$, $\mathrm{span}(S) = \{ \sum_{i=1}^q \alpha_i x_i : \alpha_i \in \mathbb{R} \}$.
%Let $\mathbbm{1}_X$ be the indicator function of $X$, i.e. $\mathbbm{1}_X = 1$ if $X$ is true and 0 otherwise.

==> main/latexmkrc.tex <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> main/our_model.tex <==
\label{sec:modelFormulation}
% One standard way to approach the problem of learning a ranking on $n$ items is to assume each item has a utility associated to it as done in the Bradley-Terry-Luce model for pairwise comparisons and Placket-Luce model for $k$-wise comparisons. The underlying ranking on the items is obtained by ranking the items by their utility and given a set of $k$ items, the distribution of observing a particular $k$-wise comparisons is parameterized by these utilities. 

% When each item $i$ has a set of features $U_i \in \mathbb{R}^d$, one typical way to produce a utility for each item is to assume there exists $w^* \in \mathbb{R}^d$ so that the utility of item $i$ is $\langle U_i, w^* \rangle$. \todo{should I remove the above two paragraphs since it's just restating what's in the related work?}

% In contrast, given a set of $k$ items, our threshold preference model assumes the utilities assigned to the items depends on the $k$-items being compared. In particular, we assume there exists $w^* \in \mathbb{R}^d$ so that given a set of $k$ items $T$, only $\Omega_T \subseteq [d]$ of the features are used to assign utilities to each of the items $i \in T$: $\langle U_i^{\Omega_T}, w^* \rangle$. These utilities can be interpreted as humans projecting the features of the items onto a smaller subspace spanned by the coordinates of $\Omega_T$ and then performing their comparative judgments in this smaller subspace.

% These utilities capture the assumption that humans will generally only use features that ``stand out'' to them to make their comparison judgments. We also assume that if humans could rank every item at the same time, they would incorporate every feature into their comparative decisions since when there are many items it is less likely that one feature will ``stand out.'' \todo{too informal?} Therefore, the ultimate goal is to rank all the items by the utilities that utilize all the features: $\langle U_i, w^* \rangle$. With knowledge of the features of each item $U_i$, we can estimate $w^*$ with maximum likelihood estimation. In the next subsection, we formalize the threshold preference model and in the subsequent subsection we formalize maximum likelihood estimation.

%Our formulation will have the property that for large $k$ each feature will likely ``stand out'' equally the same and thereby resulting in utilizing most features in the $k$-wise comparison.

%  The threshold preference model is a probabilistic model for $k$-wise comparisons on a set of items where the $k$-wise comparisons may not necessarily . What differentiates the threshold model from standard discrete choice models like the Bradley-Terry-Luce or Placket-Luce model is the where the items have features and the features used in the $k$-wise comparison are dependent on the items being compared.  when $k$ is small, there may be a handful of prominent features that ``stand out'' as opposed to when $k$ is large all the features may be used since most features will have the same variation. Given a set of items, instead of taking into account and weighing every feature that appears, people will only use some features which is effectively projecting the features onto a smaller subspace. In this work, we apply this idea to the Placket-Luce model for discrete choice. 

\paragraph{Salient Feature Preference Model}
%\label{subsec:salientModel}
%Suppose there are $n$ items such that $U_i \in \mathbb{R}^d$ are the features of item $i$ for $i \in [n]$. Let $U := \begin{bmatrix} U_1 U_2 \cdots U_n \end{bmatrix} \in \mathbb{R}^{d \times n}$ where $U_{ij}$ denotes the $i,j$-th of $U$ entry. Let $w^* \in \mathbb{R}^d$ be the \textit{judgment weights}, which signifies how important each feature is when comparing items. For $i \in [d]$ and $t \geq 0$, let $\tau_{t}: \mathcal{P}([n]) \rightarrow \mathcal{P}([d])$ be the \textit{threshold function} with \textit{threshold} $t$, which determines which features are used in a pairwise comparison and in general depends on the feature vectors $U_i$ for the items corresponding to the subset that is input to $\tau_t.$

Suppose there are $n$ items, and each item $j \in [n]$ has a known feature vector $U_j \in \mathbb{R}^d$. Let $U := \begin{bmatrix} U_1 U_2 \cdots U_n \end{bmatrix} \in \mathbb{R}^{d \times n}$.
%where $U_{ij}$ denotes the $i,j$-th entry of $U$. 
Let $w^* \in \mathbb{R}^d$ be the unknown \textit{judgment weights}, which signify the importance of each feature when comparing items. Let $\tau: [n] \times [n] \rightarrow \mathcal{P}([d])$ 
%let $\tau_{t}: \mathcal{P}([n]) \rightarrow \mathcal{P}([d])$ 
be the known \textit{selection function} that determines which features are used in each pairwise comparison. Let $P := \{(i,j) \in [n] \times [n]: i <j \}$ be the set of all pairs of items. %and in general depends on the feature vectors $U_i$ for the %items corresponding to the subset of size two that is 
%pair of items input to $\tau.$ 
Let $S_m = \{(i_\ell, j_\ell, y_\ell)\}_{\ell =1}^m $ be a set of $m$ independent pairwise comparison samples where $(i_\ell, j_\ell) \in P$ are chosen uniformly at random from $P$ with replacement, and $y_\ell \in \{0,1\}$ indicates the outcome of the pairwise comparison where 1 indicates item $i_\ell$ beat item $j_\ell$ and 0 indicates item $j_\ell$ beat item $i_\ell$. We model $y_\ell \sim \text{Bern}(\mathbb{P}(i_\ell >_B j_\ell))$ where
\begin{align}
\label{eq:thresholdBTL}
    \mathbb{P}(i_{\ell} >_B j_{\ell} ) = \frac{  \exp \left(\langle U_{i_{\ell}}^{\tau(i_{\ell},j_{\ell})} - U_{j_{\ell}}^{\tau(i_{\ell},j_{\ell})} , w^{*} \rangle \right)  }{ 1 + \exp \left(\langle U_{i_{\ell}}^{\tau(i_{\ell},j_{\ell})} - U_{j_
    \ell}^{\tau(i_{\ell},j_{\ell})}, w^{*} \rangle \right)}.
\end{align}
To understand the probability model given by Equation \eqref{eq:thresholdBTL}, note that $ \langle U_{i}^{\tau(i,j)}, w^{*} \rangle$ is the inner product of $U_i$ and $w^*$ after $U_i$ is projected to the coordinate subspace given by $\tau(i,j).$ Therefore, Equation \eqref{eq:thresholdBTL} is simply the utility model of Equation \eqref{eq:BTL} where the utilities are inner products computed in the subspace defined by the selection function $\tau$. If the selection function returns all the coordinates, i.e. $\tau(i,j) = [d]$, then Equation \eqref{eq:thresholdBTL} becomes the standard BTL model where the utility of item $i$ is $\langle U_i, w^*\rangle$ and fixed regardless of context, i.e., regardless of which pair is being compared. \new{This model is typically called ``BTL with features," and we will refer to it as FBTL.} See Section \ref{appendix:PLextension} in the Supplement for a natural extension of Equation \eqref{eq:thresholdBTL} to $k$-wise comparisons for $k>2$. Furthermore, we assume that the true ranking of all the items depends on all the features and is given by sorting the items by $\langle U_i, w^* \rangle$ for $i \in [n]$.

%Given a pair of items $i$ and $j$, Equation \eqref{eq:thresholdBTL} says to first project the features of the items, $U_{i}$ and $U_{j}$, onto the subspace spanned by the coordinates given by $\tau(i,j)$. Then assign a utility to each of the items by the inner product of the projected features with $w^*$:  $ \langle (U_{k})^{\tau(i,j)}, w^{*} \rangle$ for $k \in i,j$. 

% For $k \in [n]$, we collect $m$ independent $k$-wise comparisons $S^k_m = \{(T_{\ell}, \sigma_\ell) \}_{\ell = 1}^m$ by first uniformly picking a set $T_{\ell} = \{ t_1, \dots, t_k\}$ of $k$ items from all subsets of size $k$ and then picking a ranking $\sigma_\ell = (t_1, \dots, t_k)$ of the items in $T_\ell$ where
% \begin{align}
% \label{eq:thresholdPL}
%     \mathbb{P}(t_1 > \cdots > t_k ) = \prod_{\ell = 1}^k \frac{  \exp \left(\langle U_{t_\ell}^{\tau_{t}(T_\ell)}, w^{*} \rangle \right)  }{ \sum_{j \in [k] \textbackslash [\ell-1]} \exp \left(\langle U_{t_j}^{\tau_{t}(T_\ell)}, w^{*} \rangle \right)}.
% \end{align}

% We explain Equation \eqref{eq:thresholdPL}: Given a set of items $T$, first project each items' features $U_i$ for $i \in T$ onto the subspace spanned by the coordinates given by $\tau_{t}(T)$. Then utility each item by exponentiating its dot product with $w^*$: $\exp \left ( \langle (U_{t_\ell})^{\tau_{t}(T_\ell)}, w^{*} \rangle \right)$. The higher the utility an item has, the more likely the item will be ranked higher among the items in $T$. Now imagine a bag of balls where each ball corresponds to one of the items in $T$. We select balls from this bag without replacement where the probability of picking a ball is the ratio of its utility to the sum of the utilities of all the remaining balls. The order in which we select balls results in a ranking of the $k$ items. This process is what Equation \eqref{eq:thresholdPL} represents. \todo{this is already in the related work, so take it out from either here or there}

% In the pairwise comparison case ($k=2$) for two items $T_\ell = i,j$, Equation \eqref{eq:thresholdPL} reduces to
\paragraph{Selection Function}
%\label{subsec:specificThreshold}

We propose a selection function $\tau$ inspired by the social science literature, which posits that violations of rational choice axioms arise in certain scenarios because people make comparison judgments on a set of items based on the features that differentiate them the most \cite{rieskamp2006extending, brown2009enquiry, bordalo2013salience}.

%We base our model on the following theory from the social science literature:
% \begin{quote}
% When people compare multiattribute options, the similarity of values along one attribute enhances differences on other attributes. These comparability effects are easily linked to cognitive processing. When evaluating options, people pay more attention to attributes that differ. \cite{rieskamp2006extending}.
% \end{quote} 
% Let \begin{align}
%     \bar{s}(\{x_1, \dots, x_n\}) := \frac{1}{n} \sum_{i = 1}^n (x_i - \bar{x})
% \end{align} \todo{make this for pairs}
For two variables $w, z \in \mathbb{R}$, let $\mu := (w+z)/2$ be their mean and $\bar{s} := ((w - \mu)^2 + (z - \mu)^2)/2$ be their sample variance. Given $t \in [d]$ and items $i, j \in [n]$, the \textit{top-$t$ selection function} selects the $t$ coordinates with the $t$ largest sample variances in the entries of the feature vectors $U_i$, $U_j$.

\paragraph{Algorithm: Maximum Likelihood Estimation}
Given observations $S_m = \{(i_\ell, j_\ell, y_\ell)\}_{\ell =1}^m $, item features $U \in \mathbb{R}^{d \times n}$, and a selection function $\tau$, the negative log-likelihood of $w \in \mathbb{R}^d$ is 
% \begin{align}
%   &  \mathcal{L}_{m}(w; U, S_m, \tau ) \\
%     & = \sum_{\ell = 1}^m \log\left(1+\exp\left( \left\langle w, U_{i_\ell}^{\tau(i_\ell,j_\ell)} - U_{j_\ell}^{\tau(i_\ell,j_\ell)} \right\rangle \right) \right) - y_\ell   \left\langle w, U_{i_\ell}^{\tau(i_\ell,j_\ell)} - U_{j_\ell}^{\tau(i_\ell,j_\ell)} \right\rangle,
%     \label{eq:logLoss}
% \end{align}

\begin{align}
    \mathcal{L}_{m}(w; U, S_m, \tau ) = \sum_{\ell = 1}^m \log\left(1+\exp\left( u_{i_{\ell},j_{\ell}} \right) \right) - y_\ell   u_{i_{\ell},j_{\ell}},
    \label{eq:logLoss}
\end{align}
where $u_{i_{\ell},j_{\ell}} = \left\langle w, U_{i_\ell}^{\tau(i_\ell,j_\ell)} - U_{j_\ell}^{\tau(i_\ell,j_\ell)} \right\rangle.$

Equation \ref{eq:logLoss} is equivalent to logistic regression with features $x_\ell = U_{i_\ell}^{\tau(i_{\ell},j_{\ell})} - U_{j_\ell}^{\tau(i_{\ell},j_{\ell})}$. See Section \ref{appendix:LLderiv} of the Supplement for the derivation. We estimate $w^*$ with the maximum likelihood estimator $\hat{w}$, which requires minimizing a convex function:
$\hat{w} := \text{argmin}_{w} \mathcal{L}_m(w; U, S_m, \tau).$


% \begin{algorithm}[H]
%     \SetAlgoLined
%     \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%     \Input{ $U$ the features of the $n$ items, 
%     $\tau$ a selection function,
%     $S_m$ a set of i.i.d. pairwise comparison samples, and $\Theta \subseteq \mathbb{R}^d$}
%     \Output{$\hat{w} := \text{argmin}_{w \in \Theta} \mathcal{L}_m(w; U, S_m, \tau)$}
% \caption{Maximum likelihood estimation of $w^*$ under the salient feature preference model}
% \label{alg:MLE}
% \end{algorithm}

% We remark that the salient feature preference model has a connection to dropout \cite{srivastava2014dropout}. First notice that the salient feature preference model is a logistic regression model where the features are differences of vectors $\{U_i^{\tau(i,j)} - U_j^{\tau(i,j)}\}$ and where the binary labels are the outcomes of the pairwise comparisons. Also notice logistic regression can be viewed as a neural network with no hidden layers and with sigmoid activation on the output. Now suppose the selection function is random and picks each coordinate independently with some probability for each pair of items. Then solving for the MLE of the salient feature preference model with this random selection function is similar to using dropout to solve the MLE of BTL with features, i.e. Equation \eqref{eq:BTL} where $u_i = \langle U_i, w^* \rangle$ for $i \in [n]$ .


==> main/synthetic_experiments.tex <==
We investigate violations of rational choice arising from the salient feature preference model and illustrate Theorem \ref{thm:sampleComplexity} while highlighting the differences between the salient feature preference model and the FBTL model throughout. Given the very reasonable simulation setup we use, these experiments suggest that the salient feature preference model may sometimes be better suited to real data than FBTL.
%We present results on the top-$t$ selection function. 
%See Section \ref{appendix:figs} of the Supplement for the corresponding experiments for the RISV selection function.

For these experiments, the ambient dimension $d=10$, the number of items $n = 100$, and comparisons are sampled from the salient feature preference model with top-$t$ selection function. The coordinates of $U$, respectively $w^*$, are drawn from %$\mathcal{N}\left(0, \frac{1}{\sqrt{d}}\right)$, 
$\mathcal{N}(0, 1/\sqrt{d})$, respectively
$\mathcal{N}(0, 4/\sqrt{d})$, so that $\mathbb{P}(i>_B j)$ is bounded away from $0$ and $1$ for $i,j \in [n]$. This set-up ensures $b^*$ does not become too large.

First, the salient feature preference model can produce preferences that systematically violate rational choice. In contrast, the FBTL model cannot. Let $P_{ij} = \mathbb{P}(i>_B j)$ and $T = \{ (i,j,k) \in [n]^3: P_{ij} > .5, P_{jk} > .5\}$. Then $(i,j,k) \in T$ satisfies strong stochastic transitivity if $P_{ik}\geq \max\{P_{ij}, P_{jk} \}$, moderate stochastic transitivity if $P_{ik} \geq \min\{P_{ij}, P_{jk} \}$, and weak stochastic transitivity if $P_{ik} \geq .5$ \cite{cattelan2012models}. We sample $U$ and $w^*$ 10 times as described in the beginning of the section and allow $t$ to vary in $[d]$. Figure \ref{fig:violationRationalChoice} shows the average ratio of the number of weak, moderate, and strong stochastic transitivity violations to $|T|$ as a function of $t \in [d]$. There is very little deviation from the average. The standard error bars over the 10 experiments were plotted but they are so small that the markers covered them. All $\binom{n}{2}$ probabilities given by Equation \eqref{eq:thresholdBTL} are used to calculate the intransitivity rates. In the same figure we also show the percentage of pairwise comparisons that are inconsistent with the true ranking under the same experimental set-up. These are the pairs $i,j$ such that $\langle U_{i} - U_{j}, w^* \rangle < 0$, meaning item $i$ is ranked lower than item $j$ in the true ranking, but $\langle U_{i}^{\tau_{t}(i,j)} - U_{j}^{\tau_{t}(i,j)}, w^* \rangle >0$ meaning item $i$ beats item $j$ by at least 50\% when compared in isolation from the other items.
%
%Furthermore, the salient feature preference model produces pairwise comparisons that are inconsistent with the underlying true ranking. Consider items $i,j$ such that $\langle U_{i} - U_{j}, w^* \rangle < 0$, meaning item $i$ is ranked lower than item $j$ in the true ranking. This pair may be such that $\langle U_{i}^{\tau_{t}(i,j)} - U_{j}^{\tau_{t}(i,j)}, w^* \rangle >0$ meaning item $i$ beats item $j$ by at least 50\% when compared in isolation from the other items. In Figure \ref{fig:violationRationalChoice}, we also show the percentage of pairwise comparisons that are inconsistent with the true ranking under the same experimental set-up as before. 
Notice that when $t=10$, the salient feature preference model is the FBTL model, so there are no pairwise inconsistencies or intransitives. Although this example is synthetic, real data exhibits intransitivity and even inconsistent pairs with the underlying ranking as discussed in the real data experiments in Section \ref{sec:realDataExp}. 

%Pairwise inconsistencies can be viewed as a type of preference reversal \cite{lichtenstein1971reversals}.  
\begin{figure}%
    \centering
    \includegraphics[width=7.5cm]{main/figs/synthetic_experiment_figs/sst_sst_pi.pdf}
    \caption{The salient feature preference model with the top-$t$ selection function produces systematic intransitives and pairwise comparisons that are inconsistent with the underlying ranking. When $t=10$, the salient feature preference model with the top-$t$ selection function is the FBTL model, and hence there are no intransitives or pairwise inconsistencies.}
    \label{fig:violationRationalChoice}
\end{figure}

Second, we illustrate Theorem \ref{thm:sampleComplexity} with the top-$1$ selection function, and where $U$ and $w$ are sampled once as described in the beginning of this section. We sample $m$ pairwise comparisons for $m \in \{(100)2^{i-1}: i \in [10]\}$, fit the MLEs of both the salient preference model with the top-$1$ selection function and FBTL, and repeat 10 times. Figure \ref{fig:varySamples} shows the average estimation error of $w^*$ on a logarithmic scale as a function of the number of pairwise comparison samples also on a logarithmic scale. Figure \ref{fig:varySamples} also shows the exact theoretical upper bound where $\delta = \frac{1}{d} = \frac{1}{10}$ of Theorem \ref{thm:sampleComplexity} without constants $C_1$ and $C_2$ as stated in Section \ref{appendix:sampleComplexityProof} of the Supplement.
%: $$\frac{4(1 + \exp(b^*))^2}{\exp(b^*)\lambda}  \sqrt{\frac{3\beta^2\log{(2d^2)}d + 4\sqrt{d}\beta \log{(2d^2)}}{6m}}.$$
Again, there is very little deviation from the average. The standard error bars over the 10 experiments were plotted but they are so small that the markers covered them. % Since $U$ and $w^*$ are fixed, the bound is valid for the entire experiment. 
There is a gap between the observed error and the theoretical bound, though the error decreases at the same rate. 
%Furthermore, $m_1 \approx 130 $ and $m_2 \approx 4300$ where $m_1$ and $m_2$ are defined in Theorem \ref{thm:sampleComplexity}.
The error of the MLE of FBTL does not improve with more samples, since the pairwise comparisons are generated according to the salient feature preference model with the top-$1$ selection function. 
\begin{figure}%
    \centering
    \includegraphics[width=7.5cm]{figs/synthetic_experiment_figs/error.pdf}
    \caption{Illustration of Theorem \ref{thm:sampleComplexity} with the exact theoretical upper bound for the salient feature preference model with the top-$1$ selection function. Although there is a gap between the bound and the observed estimation error, they decrease at the same rate eventually. Excluding the first two points, the salient feature MLE error’s slope on the log-log scale is -0.154, whereas the theoretical bound’s slope is -0.151.}
    \label{fig:varySamples}%
\end{figure} See Section \ref{sec:additionalExperiments} in the Supplement for investigating model misspecification, i.e. fitting the MLE of the top-$t$ selection function for $t \neq 1$ with the same experimental set-up. 

 By estimating $w^*$ well, we can estimate the underlying ranking well by Corollary \ref{coro:rankingComplexity}. Under the same experimental set up, Figure \ref{fig:ktError} shows the Kendall tau correlation (definition given in Supplement \ref{sec:additionalExperiments}) between the true ranking (obtained by ranking the items according to $\langle U_i, w^* \rangle$) and the estimated ranking (according to $\langle U_i, \hat{w} \rangle$) but on a new set of 100 items drawn from the same distribution. %Let $\gamma, \rho: [n] \rightarrow [n]$ be two rankings on $n$ items where $\gamma(i)$ and $\rho(i)$ is the position of item $i$ in the ranking. Let $A = \sum_{(i,j) \in P} \mathbbm{1}_{\{(\sigma(i) - \sigma(j))(\rho(i) - \rho(j))>0\}}$, respectively $D = \sum_{(i,j) \in P} \mathbbm{1}_{\{(\sigma(i) - \sigma(j))(\rho(i) - \rho(j))\leq 0\}} $,  be the number of pairs of items that $\sigma$ and $\rho$ agree, respectively disagree, on the relative ordering. Then the Kendall tau correlation of $\rho$ and $\gamma$ is $KT(\gamma, \rho):=\frac{A-D}{\binom{n}{2}}$.
 %Note $\mathrm{KT}(\sigma,\rho) = 1$ when $\sigma = \rho$, and $\mathrm{KT}(\sigma,\rho) = 0$ means $\sigma$ and $\rho$ agree on the same number of pairwise comparisons as they disagree on. 
The maximum Kendall tau correlation between two rankings is 1 and occurs when both rankings are equal.  Also, estimating $w^*$ well allows us to predict the outcome of unseen pairwise comparisons well, as shown in the Supplement in Section \ref{sec:additionalExperiments}. %The definition of Kendall tau correlation is also given in that section for completeness.

\begin{figure}%
    \centering
    \includegraphics[width=7.5cm]{figs/synthetic_experiment_figs/kt_error.pdf}
    \caption{Kendall tau correlation between the true ranking and the estimated ranking where pairwise comparisons are sampled from the salient feature preference model with the top-$1$ selection function. Estimating $w^*$ well implies being able to estimate the underlying ranking well as stated in Corollary \ref{coro:rankingComplexity}.}
    \label{fig:ktError}%
\end{figure} 




==> main/synthetic_experiments_old.tex <==
We highlight the differences between the salient feature preference model and the FBTL model, investigate violations of rational choice arising from the salient feature preference model, and illustrate Theorem \ref{thm:sampleComplexity}. Given the very reasonable simulation setup we use, these experiments suggest that the salient feature preference model may sometimes be better suited to real data than the FBTL model. We present results on the top-$t$ selection function. 
%See Section \ref{appendix:figs} of the Supplement for the corresponding experiments for the RISV selection function.

First, under the salient feature preference model, we investigate the affect of the threshold of the RASV selection function on learning $w^*$ and the underlying ranking. We set $n = 200$, $d = 20$, $m = 10,000$, and sample columns of $U \in \mathbb{R}^{d \times n}$ from a Gaussian mixture model $\sum_{i = 1}^4 \frac{1}{4} \mathcal{N}(\mu_i,I)$ where $\mu_i \sim N(0, \sqrt{3}I)$, and $w \in \mathbb{R}^d \sim \mathcal{N}(0,I)$ and normalized to have unit norm. For a fixed $U$ and $w$, 10,000 pairwise comparisons are sampled from the salient feature preference model of Equation \eqref{eq:thresholdBTL} with the RASV selection function of Equation \eqref{eq:AVT} with threshold $t \in \{.05, .1, \dots, .95, 1\}$. This procedure is repeated 10 times with a new $U$ and $w$. 


The first plot in Figure \ref{fig:syntheticExperiments} shows the average estimation error of $w^*$ on the logarithmic scale, i.e. $\frac{1}{10} \sum_{i=1}^{10} \log_{10}(\|w^* - \hat{w}_i\|_2 )$, and the standard deviation of the MLE of the salient feature preference model with the RASV selection function and the BTL model. The second plot in Figure \ref{fig:syntheticExperiments} shows the Kendall tau correlation between the true ranking (obtained by ranking the items according to $\langle U_i, w^* \rangle$) and the estimated ranking (according to $\langle U_i, \hat{w} \rangle$). The Kendall tau correlation between two rankings $\sigma, \rho: [n] \rightarrow [n]$ on $n$ items, where $\sigma(i)$ is the position of item $i$ in the ranking, is defined as
\begin{align}
    \text{KT}(\sigma, \rho) = \frac{\sum_{(i,j) \in P} \mathbbm{1}_{\{(\sigma(i) - \sigma(j))(\rho(i) - \rho(j))>0\}} - \sum_{(i,j) \in P} \mathbbm{1}_{\{(\sigma(i) - \sigma(j))(\rho(i) - \rho(j))\leq 0\}} }{\binom{n}{2}}.
\end{align}
$\mathrm{KT}(\sigma,\rho) = 1$ when $\sigma = \rho$, and $\mathrm{KT}(\sigma,\rho) = 0$ means $\sigma$ and $\rho$ agree on the same number of pairwise comparisons as they disagree on. 
%The ranking obtained by the BTL MLE without features estimates the ranking more poorly than the BTL with features MLE since it is not utilizing the item features. 
%Although Theorem \ref{thm:sampleComplexity} does not imply that the Kendall tau correlation of the resulting ranking obtained by the MLE of $w^*$ and the true ranking will converge to 1, we see that the MLE produces a ranking that is close to the true ranking. \todo{take this sentence out?}
For every threshold $t < 1$, there is a gap between the estimation error of $w^*$ (and the Kendall tau correlation) under the MLE of the salient feature preference model and the MLE of the BTL model, illustrating that the salient feature preference model is quantitatively different than the BTL model though we remark that this gap is expected since the synthetic preference data is generated with respect to the RASV model, not the BTL model. Furthermore, we expect that as the threshold increases, the gap between the two models improves since the RASV model -- which is how the data is generated -- becomes more and more like the BTL model since more and more features will be used in each context-dependent comparison.

\begin{figure}%
    \centering
    \includegraphics[width=14cm]{figs/synthetic_experiment_figs/w_error_KT_RASV.pdf}
    \caption{First two figures: For 10,000 samples from the salient feature preference model with the RASV selection function, there is a significant gap between the MLE of the BTL model and the salient feature preference model on the estimation error of $w^*$ and the Kendall tau correlation of the estimated ranking with the true ranking. Last figure: Illustration of Theorem \ref{thm:sampleComplexity} for the salient feature preference model under the RASV selection function with threshold $t = .4$.}
    \label{fig:syntheticExperiments}%
\end{figure}

%Third figure: systematic intransitives arise under the same sampling model of the first two plots.

% \begin{figure}%
%     \centering
%     \subfloat{{\includegraphics[width=5cm]{synthetic_experiment_figs/w_error_threshold_sweep_indp.pdf}
%     }}%
%     \subfloat{{\includegraphics[width=5cm]{synthetic_experiment_figs/w_error_threshold_sweep_indp.pdf} }}%
%     \caption{2 Figures side by side}%
%     \label{fig:example}%
%     \subfloat{{\includegraphics[width=5cm]{synthetic_experiment_figs/w_error_threshold_sweep_indp.pdf}
%     }}%
%     \subfloat{{\includegraphics[width=5cm]{synthetic_experiment_figs/w_error_threshold_sweep_indp.pdf} }}%
%     \caption{2 Figures side by side}%
%     \label{fig:example}%
% \end{figure}

%\includegraphics[width=7cm]{synthetic_experiment_figs/w_error_threshold_sweep_additive.pdf}

% \begin{figure}%
%     \centering
%     \subfloat[test]{{\includegraphics[width=8cm]{synthetic_experiment_figs/w_KT_additive.pdf} }}%
%     \qquad
%     \subfloat[label 2]{{\includegraphics[width=5cm]{synthetic_experiment_figs/w_error_threshold_sweep_additive.pdf} }}%
%     \caption{2 Figures side by side}%
%     \label{fig:example}%
% \end{figure}
%As the threshold increases, the estimation error of $w^*$ decreases and similarly the Kendall tau correlation increases. 
%The MLE of the BTL model struggles much more with intransitivity and pairwise comparisons that are inconsistent with the underlying ranking. 

%and while our salient feature preference model can handle these issues, it will require more samples to learn $w^*$ well the more these issues are present. When the threshold is equal to 1, both the BTL with features model and our salient feature preference model are equivalent since all the features are utilized in the utilities. \todo{LKB took this out because of course we can learn w* when it follows our likelihood model and we have enough data. The point is more that BTL does not still do fine.}
 \todo{should i comment about why the blue line in the left plot is not perfectly monotonic?}
\todo{should i comment about how the red line on the left side plot has small variance, but large variance on the right handside? I guess this says that the BTL MLE estimator produces utilities that are very close.}

% Our salient feature preference model results in pairwise comparisons that violate properties that pairwise comparisons drawn from a standard BTL model must satisfy. Since these properties likely dictate the difficulty of learning $w^*$, we plot these properties. We use all pairs and the exact pairwise probabilities instead of empirical. We depict the average and standard deviation over the 10 trials with the same 10 $U$ and $w$ from the previous experiment.

Second, the salient feature preference model produces preferences that systematically violate rational choice, which can explain why the MLE of the BTL model struggles to estimate $w^*$ since BTL fundamentally cannot model these violations. Let $P_{ij} = \mathbb{P}(i>j)$ and $T = \{ (i,j,k) \in [n]^3: P_{ij} \geq .5, P_{jk}\geq.5\}$, then $(i,j,k) \in T$ satisfies strong stochastic transitivity if $P_{ik}\geq \max\{P_{ij}, P_{jk} \}$, moderate stochastic transitivity if $P_{ik} \geq \min\{P_{ij}, P_{jk} \}$, and weak stochastic transitivity if $P_{ik} \geq .5$ \cite{cattelan2012models}. The first plot in Figure \ref{fig:propsRASV} shows the average ratio of the number of weak, moderate, strong stochastic transitivity violations to $|T|$ with the standard deviation from the the same ten $U$ and $w$ from the previous experiment where we use all of the exact pairwise probabilities given by the salient feature preference model under the RASV selection function. Furthermore, the salient feature preference model produces pairwise comparisons that are inconsistent with the underlying true ranking. Consider items $i,j$ such that $\langle U_{i} - U_{j}, w^* \rangle < 0$, meaning item $i$ is ranked lower than item $j$ in the ranking. This pair may be such that $\langle U_{i}^{\tau_{t}(i,j)} - U_{j}^{\tau_{t}(i,j)}, w^* \rangle >0$ meaning item $i$ beats item $j$ by at least 50\% when compared in isolation from the other items. See the second plot in Figure \ref{fig:propsRASV}, which shows what percentage of pairwise comparisons of all pairwise comparisons are inconsistent with the true ranking under the same set-up of the intransitivity results. Although a synthetic example, real data exhibits intransitivity and inconsistent pairs with the underlying ranking as shown in the real data experiments.

\begin{figure}%
    \centering
    \includegraphics[width=12cm]{figs/synthetic_experiment_figs/rational_violation_RASV.pdf}
    \caption{The salient feature preference model with the RASV selection function produces systematic intransitives and pairwise comparisons that are inconsistent with the underlying ranking.}
    \label{fig:propsRASV}
\end{figure}

% Second, 

% Third, Figure \ref{fig:syntheticExperiments} also shows the low noise violation rate which is the fraction of pairs for which the low noise condition does not hold. The low noise condition is a property of the underlying pairwise probabilities and is defined as the following implication: if for any pair of items $(i,j)$ $P_{ij} > .5$, then $\sum_{k} P_{ki} > \sum_{k} P_{kj}$. The low noise condition is a sufficient condition for the MLE of the BTL without features model to produce a ranking that minimizes the number of pairs that disagree with the underlying ranking \cite{rajkumar2016can}.

% Since the salient feature preference model only uses some features for each pairwise comparison, we consider how many features on average are used by each pairwise comparison. See Figure \ref{fig:syntheticExperiments}. Other than when the threshold is 1, no sampled pairwise comparison utilizes all the features in the resulting utilities, i.e. $\tau_t(\{i,j\}) \neq [d].$ As one might expect, in the regime where only a few features are used is where the most intransitives and inconsistencies with the underlying ranking arise.

% \begin{figure}%
%     \centering
%     \includegraphics[width=15cm]{synthetic_experiment_figs/props_additive.pdf}
%     \caption{The effect of varying the threshold of the salient feature preference model with the RASV selection function on properties of the pairwise comparisons. This model produces a significant number of intransitive preferences and also pairwise comparisons that disagree with the underlying ranking especially for small thresholds. }%
%     \label{fig:syntheticExperiments}%
% \end{figure}

 %model in certain scenarios especially since the sampling distribution, which is a mixture of Gaussians, for $U$ is reasonable.

Finally, we illustrate Theorem \ref{thm:sampleComplexity} under the salient feature preference model with the RASV selection function with threshold $t =.4$. $U$ and $w$ are sampled once from the same distribution as before. We sample $m$ pairwise comparisons for $m \in \{1000, 5000, 10000, 25000, 50000, 75000\}$, fit the MLEs, and repeat 5 times. The last plot in Figure \ref{fig:syntheticExperiments} shows the average estimation error of $w^*$ on the logarithmic scale with the standard deviation and also the theoretical bound of Theorem \ref{thm:sampleComplexity}. Since $U$ and $w$ are fixed, the bound is valid for the entire experiment. There is a gap between the observed error and the theoretical bound, though the error decreases at the same rate. Furthermore, the number of samples required by Theorem \ref{thm:sampleComplexity} is often on the order of $10^6$ for these experiments, much greater than what we observe is required. However, the error of the MLE of BTL does not improve with more samples, likely because of the intransitives and inconsistent pairs.

% \begin{figure}%
%     \centering
%     \includegraphics[width=7cm]{synthetic_experiment_figs/w_error_threshold_sweep_additive.pdf}
%     \caption{The affect of varying the threshold on properties of the pairwise comparisons under the RASVmodel.}%
%     \label{fig:thmIllustration}%
% \end{figure}


% \begin{figure}%
%     \centering
%     \subfloat{{\includegraphics[width=9cm]{synthetic_experiment_figs/w_error_threshold_sweep_additive.pdf} }}%
%     \qquad
%     \subfloat{{\includegraphics[width=9cm]{synthetic_experiment_figs/w_error_threshold_sweep_additive_zoom.pdf} }}%
%   \caption{The affect of varying the threshold on properties of the pairwise comparisons under the RASV model.}%
%     \label{fig:thmIllustration}%
% \end{figure}
 

% First, we consider the case when all the features are used in each pairwise comparison, i.e., the threshold function $\tau_t$ is constant and always evaluates to $[d]$ where $d$ is the dimension of the features of the items. Each entry of $U \in \mathbb{R}^{d \times n}$ and $w \in \mathbb{R}^d$ is drawn from $\mathcal{N}(0,1)$ then $w$ is normalized to have unit norm. For this fixed $U$ and $w$, we sample $x \in \{2000, 4000, 6000, 8000, 10000\}$ pairwise comparisons chosen independently and uniformly at random and then find the MLE $\hat{w}$ of $w$. For each choice of number of samples, we repeat this process 5 times by sampling new pairwise comparisons and then computing $\hat{w}$. We use $d = 10$ for the dimension of the features and $n = 200$ for the number of items.

% Figure \ref{fig:thresholdAllwError} shows the average over the 5 trials of the estimation error of $w^*$  on the logarithmic scale given by $\log(\|w^* - \hat{w}\|_2 )$ with the standard deviation of the 5 trials and also the theoretical bound given by Theorem \ref{thm:sampleComplexity}. Since $U$ and $w$ are fixed, this theoretical bound holds for each of the 5 trials. In this case, the BTL with features model and the salient feature preference model are identical. We also plot the Kendall tau correlation between the true ranking obtained by ranking the items by $\langle U_i, w^* \rangle$ and also the estimated ranking by ranking the items by $\langle U_i, \hat{w} \rangle$ where the Kendall tau correlation between two rankings $\sigma, \tau: [n] \rightarrow [n]$ on $n$ items is defined as
% \begin{align}
%     \text{KT}(\sigma, \tau) = \frac{\sum_{(i,j) \in P} \mathbbm{1}_{\{(\sigma(i) - \sigma(j))(\tau(i) - \tau(j))>0\}} - \sum_{(i,j) \in P} \mathbbm{1}_{\{(\sigma(i) - \sigma(j))(\tau(i) - \tau(j))\leq 0\}} }{{n \choose 2}}
% \end{align}
% where $\sigma(i)$ is the position of item $i$ in the ranking. The ranking obtained by the BTL MLE without features has a slower convergence to the true ranking, which makes sense since it is not utilizing feature information about the items.

% \begin{figure}%
%     \centering
%     \subfloat{{\includegraphics[width=8cm]{synthetic_experiment_figs/w_error_all.pdf} }}%
%     \qquad
%     \subfloat{{\includegraphics[width=8cm]{synthetic_experiment_figs/kt_all.pdf} }}%
%     \caption{All features are used in each pairwise comparison.}%
%     \label{fig:thresholdAllwError}%
% \end{figure}

% Second, for a fixed number of samples, we use the RASVthreshold and vary the threshold to understand the role the threshold has. We generate $U$ and $w$ as we did in the first set of experiments again with $d = 10$ and $n = 200$. Then for $t \in \{.05*i: i \in [20]\}$, we sample 10,000 pairs of pairwise comparisons and fit the MLE $\hat{w}$. This procedure is repeated 5 times. 

% Figure \ref{fig:thresholdSweep} shows the estimation error of $w^*$ over each choice of threshold and the Kendall tau correlation from the true ranking to the estimated ranking. The error bars is the standard deviation over the 5 trials. As expected, as the threshold increases, the salient feature preference model and the BTL with features model converge to the same model.
% % 

% \begin{figure}%
%     \centering
%     \subfloat{{\includegraphics[width=9cm]{synthetic_experiment_figs/w_error_threshold_sweep.pdf} }}%
%     \qquad
%     \subfloat{{\includegraphics[width=9cm]{synthetic_experiment_figs/kt_threshold_sweep.pdf} }}%
%     \caption{The affect of threshold when using RASVthreshold.}%
%     \label{fig:thresholdSweep}%
% \end{figure}

% What makes the salient feature preference model fundamentally different from the BTL model is that the salient feature preference model allows pairwise comparisons that disagree with the underlying true ranking, i.e., the salient feature preference model can model a pair of items for which $\langle U_{i}^{\tau_{t}(\{i,j\})} - U_{j}^{\tau_{t}(\{i,j\})}, w^* \rangle >0$ meaning item $i$ beats item $j$ with probability greater than 50\% when only compared to themselves yet $\langle U_{i} - U_{j}, w^* \rangle \leq 0$ meaning item $i$ is lower in the ranking than item $j$ when incorporating all features into the ranking judgment. See Figure \ref{fig:inconsistenciesThresholdSweep} that shows what percentage of pairwise comparisons over all pairwise comparisons disagree with the underlying true ranking for each choice of threshold. Similarly, the preference model can result in intransitives. One way to measure intransitivity in ranking data is to consider triplets of items $(i,j,k)$ \cite{cattelan2012models}. A triplet satisfies strong stochastic transitivity if $P_{ij} > .5$ and $P_{jk}>.5$ implies $P_{ik}> \max\{P_{ij}, P_{jk} \}$. A triplet satisfies moderate stochastic transitivity if if $P_{ij} > .5$ and $P_{jk}>.5$ implies $P_{ik}> \min\{P_{ij}, P_{jk} \}$. And finally a triplet satisfies weak stochastic transitivity if if $P_{ij} > .5$ and $P_{jk}>.5$ implies $P_{ik}> .5$. Out of all possible triplets, we record how many satisfies $P_{ij} > .5$ and $P_{jk}>.5$ and call this the number of valid triplets. Figure \ref{fig:intransitivitiesThresholdSweep} shows how the ratio of the number of weak, moderate, strong and the number of valid triplets changes as the threshold changes.

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/st_threshold_sweep.pdf}
%     \caption{The affect of varying the threshold on intransitivity for the RASVthreshold.}%
%     \label{fig:intransitivitiesThresholdSweep}%
% \end{figure}

% We also plot the low noise violation rate which is the fraction of pairs for which the low noise condition does not hold. See Figure \ref{fig:LNThresholdSweep}. The low noise condition is a property of the underlying pairwise probabilities and is defined as the following: if for any pair of items $(i,j)$ $P_{ij} > .5$, then $\sum_{k} P_{ki} > \sum_{k} P_{kj}$. The low noise condition is a sufficient condition for the MLE of the BTL without features model to produce a ranking that minimizes the number of pairs that disagree with the underlying ranking \cite{rajkumar2016can}.

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/inconsistency_threshold_sweep.pdf}
%     \caption{The affect of varying the threshold on pairwise inconsistency rate for the RASVthreshold.}%
%     \label{fig:inconsistenciesThresholdSweep}%
% \end{figure}

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/LN_threshold_sweep.pdf}
%     \caption{The affect of varying the threshold on low noise for the RASVthreshold.}%
%     \label{fig:LNThresholdSweep}%
% \end{figure}

% Since the salient feature preference model only uses some features for each pairwise comparison, it is interesting to see how many features on average each pairwise comparison uses. See Figure \ref{fig:avgNumFeaturesAndSat}.

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/avg_h_threshold_sweep.pdf}
%     \caption{The affect of varying the threshold on how many features are used in a pairwise comparison for the RASVthreshold.}%
%     \label{fig:avgNumFeaturesAndSat}%
% \end{figure}

% In order to illustrate Theorem \ref{thm:sampleComplexity}, for the threshold set to $t = .1$ and $t = .8$, we plot the estimation error of $w^*$ along with the predicted theoretical bound in Figure \ref{fig:thresholdSampleComplexity}.

% \begin{figure}%
%     \centering
%     \subfloat{{\includegraphics[width=8cm]{synthetic_experiment_figs/w_error_2_additive_thresh.pdf} }}%
%     \qquad
%     \subfloat{{\includegraphics[width=8cm]{synthetic_experiment_figs/kt_2_additive_thresh.pdf} }}%
%     \caption{RASVthreshold function with threshold $t = .2$}%
%     \label{fig:thresholdSampleComplexity}%
% \end{figure}

% We repeat the above experiments for the relative independent sample variance threshold function. 

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/w_error_threshold_sweep_indp.pdf}
%     \label{fig:wErrorThresholdSweepIndp}%
%     \caption{The affect of the threshold on estimation error under the relative independent sample variance threshold.}
% \end{figure}

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/kt_threshold_sweep_indp.pdf}
%     \label{fig:ktErrorThresholdSweepIndp}%
%     \caption{The affect of the threshold on estimated ranking with the relative independent sample variance threshold.}
% \end{figure}

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/st_threshold_sweep_indp.pdf}
%     \caption{The affect of the threshold on transitivity properties with the relative independent sample variance threshold.}
%     \label{fig:stThresholdSweepIndp}%
% \end{figure}

% \begin{figure}%
%     \centering
% \includegraphics[width=8cm]{synthetic_experiment_figs/LN_threshold_sweep_indp.pdf}
%     \caption{The affect of the threshold on low noise violations with the relative independent sample variance threshold.}
%     \label{fig:LNThresholdSweepIndp}%
% \end{figure}

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/avg_h_threshold_sweep_indp.pdf}
%     \caption{The affect of the threshold on how many features are used on average in a pairwise comparison that does not use all features with the relative independent sample variance threshold.}
%     \label{fig:avgHThresholdSweepIndp}%
% \end{figure}

% \begin{figure}%
%     \centering
%     \subfloat{{\includegraphics[width=8cm]{synthetic_experiment_figs/w_error_2_indp_thresh.pdf} }}%
%     \qquad
%     \subfloat{{\includegraphics[width=8cm]{synthetic_experiment_figs/kt_2_indp_thresh.pdf} }}%
%     \caption{Relative independent sample variance threshold function with threshold $t = .2$}%
%     \label{fig:thresholdSampleComplexity}%
% \end{figure}


% Third we consider different models for $U$ that result in a marked difference between the salient feature preference model and the BTL with features model with respect to the learned ranking. We sample the columns of $U$ from a mixture of 3 Gaussians whose means are drawn from $\mathcal{N}(0, 2I)$ such that each Gaussian has equal chance of being drawn. We set $d = 10$ and $n=200$.

==> main/theory.tex <==
\label{sec:theory}
In this section, we analyze the sample complexity of estimating the judgment weights with the MLE given by minimizing $\mathcal{L}_m$ of Equation \eqref{eq:logLoss}. We first consider the sample complexity under an arbitrary selection function, and then specialize to two concrete selection functions: one that selects all features per pair and another that selects just one feature per pair. Throughout this section, we assume the set-up and notation presented in the beginning of Section \ref{sec:modelFormulation}.
%suppose there are $n$ items where columns of $U \in \mathbb{R}^{d \times n}$ are their features, $w^* \in \mathbb{R}^d$ is the judgment vector, and $\tau$ is the selection function. Let $S_m = \{(i_{\ell}, j_{\ell}, y_\ell)\}_{\ell = 1}^m$ be the $m$ samples of pairwise comparisons defined at the beginning of Section \ref{sec:modelFormulation}.
%where each pair of items $(i_{\ell}, j_{\ell})$ is chosen uniformly at random from all the pairs of items and $y_\ell$ is 1 if the $i_{\ell}$-th item beats the $j_{\ell}$-th item and 0 otherwise where $y_\ell \sim \text{Bernoulli}\left(\frac{  \exp \left(\langle U_{i_\ell}^{\tau_{t}(T_\ell)} - U_{j_\ell}^{\tau_{t}(T_\ell)} , w^{*} \rangle \right)  }{ 1 + \exp \left(\langle U_{i_\ell}^{\tau_{t}(T_\ell)} - U_{j_\ell}^{\tau_{t}(T_\ell)}, w^{*} \rangle \right)}\right)$. 
% $\bar{P} := [n] \times [n]$ denote all the ordered pairs of items and
%Let $P := \{(i,j) \in [n] \times [n]: i<j\}$ denote all the pairs of items. 

First, the following proposition completely characterizes the identifiability of $w^*$. Identifiability means that with infinite samples, it is possible to learn $w^*$. Precisely, the salient feature preference model is identifiable if for all $(i,j) \in P$ and for $w_1, w_2 \in \mathbb{R}^d$, if $\mathbb{P}(i >_B j; w_1 ) = \mathbb{P}(i >_B j; w_2 )$, then $w_1 = w_2$ where $\mathbb{P}(i >_B j; w)$ refers to Equation \eqref{eq:thresholdBTL} where $w$ is the judgement vector. The proof is in Section \ref{appendix:identifiability} of the Supplement.
\begin{prop}[Identifiability]
\label{prop:identifiability}
Given item features $U \in \mathbb{R}^{n \times d}$, the salient feature preference model with selection function $\tau$ is identifiable if and only if $\text{span}\{ U_i^{\tau(i,j)} - U_j^{\tau(i,j)}: (i,j) \in P \} = \mathbb{R}^d$. 
\end{prop}

Now we present our main theorem on the sample complexity of estimating $w^*$. Let 
\[b^*: = \max_{(i,j) \in P} | \langle w^*, U_i^{\tau(i,j)} - U_j^{\tau(i,j)} \rangle |,\] which is the maximum absolute difference between two items' utilities when comparing them in context, i.e. based on the features given by the selection function $\tau$. Let \[\mathcal{W}(b^*) := \{ w \in \mathbb{R}^{d}: \max_{(i,j) \in P} | \langle w, U_i^{\tau(i,j)} - U_j^{\tau(i,j)} \rangle| \leq b^* \}.\] We constrain the MLE to $\mathcal{W}(b^*)$ so that we can bound the entries of the Hessian of $\mathcal{L}_m$ in our theoretical analysis. We do not enforce this constraint in our synthetic experiments.
%While this constraint is needed for our theoretical analysis, we do not enforce this constraint in our synthetic experiments.
%Also, let $B_{U, t} := \max_{(i,j) \in P} \| U_{i}^{\tau_{t}(i,j)} - U_{j_\ell}^{\tau_{t}(i,j)} \|_{\infty}.$

% We assume the sum of the columns of $U$ is 0, which implies that the sum of the utilities of the items is 0 when taking all features into account: $\sum_{i=1}^n \langle w^*, U_i\rangle = 0$. If this assumption is not true, we subtract the sum of the columns $U$ from each column of $U$ which will not alter the distribution of the pairwise comparisons given by Equation \eqref{eq:thresholdBTL}, $b$, or $B$. \todo{this deals with identifaibility}

% Under this model for sampling, by Lemma \ref{lem:MLEObjective} in the Supplement, the average negative log likelihood of the sample pairwise comparisons given $w \in \mathbb{R}^d$ is

% \begin{equation}\label{eq:logLoss}
% \mathcal{L}_{m}(w; U, S_m, \tau ) = \frac{1}{m} \sum_{\ell = 1}^m \log\left(1+\exp \left(\langle U_{i_\ell}^{\tau_{t}(T_\ell)} - U_{j_\ell}^{\tau_{t}(T_\ell)} , w \rangle \right) \right) - y_\ell  \langle U_{i_\ell}^{\tau_{t}(T_\ell)} - U_{j_\ell}^{\tau_{t}(T_\ell)}, w \rangle.
% \end{equation} 
% We will use $\mathcal{L}_{m}(w)$ instead of $\mathcal{L}_{m}(w; U, S)$ when it is clear from context. Notice that the average negative log likelihood is convex in $w$.
 
 %Furthermore, Theorem 2 of \cite{seshadri2019discovering} is a necessary condition for identifiability of their context dependent random utility model that says identifiability implies there must be observations for $k$-wise comparisons for more than one $k$.
 %

% \begin{theorem}[Sample complexity of learning $w^*$]
% \label{thm:sampleComplexity}
% Let $U$, $w^*$, $\tau$, and $S_m$ be defined as above. Let $\hat{w}$ be the maximum likelihood estimator: $\hat{w} = \text{arg min }_{w \in \mathcal{W}(b^*)} \mathcal{L}_{m}(w; U, S_m, \tau )$. Let \[\lambda := \lambda_{\min}( \mathbb{E}((U_{i}^{\tau(i,j)} - U_{j}^{\tau(i,j)}) (U_{i}^{\tau(i,j)} - U_{j}^{\tau(i,j)})^T)).\] If $\lambda >0$ and if \[m \geq \max\left\{\frac{d}{\left(\frac{6 - \log{(2d^2)}3 dB^2}{\log{(2d^2)} 4B}\right)^2}, \frac{8\log(d)(6C + 2\lambda D_{U, \tau})}{3\lambda^2} \right\},\] then with probability at least $1 - \frac{2}{d}$ where the probability is respect to the randomly chosen pairwise comparison samples,
% \[ \| w^* - \hat{w}\|_2 \leq \frac{4(1 + \exp(b^*))^2}{\exp(b^*)\lambda} \sqrt{\frac{1}{m}}\] where $C := \|\mathbb{E}(((U_{i}^{\tau(i,j)} - U_{j}^{\tau(i,j)}) (U_{i}^{\tau(i,j)} - U_{j}^{\tau(i,j)})^T)^2)\|_2$ , $D_{U,\tau}:= \max_{(i,j) \in P} \|U_i^{\tau(i,j)} - U_j^{\tau(i,j)}\|_2^2$, and $B:=\max_{(i,j) \in P} \| U_{i}^{\tau(i,j)} - U_{j}^{\tau(i,j)} \|_{\infty}.$ In all cases, the expectation is taken with respect to a uniformly chosen random pair of items $(i, j) \in P$.
% \end{theorem}
\begin{theorem}[Sample complexity of learning $w^*$]
\label{thm:sampleComplexity}
Let $U \in \R^{d \times n}$, $w^* \in \R^d$, $\tau$, and $S_m$ be defined as in the beginning of Section \ref{sec:modelFormulation}. Let $\hat{w}$ be the maximum likelihood estimator, i.e. the minimum of $\mathcal{L}_m$ in Equation \eqref{eq:logLoss}, restricted to the set $\mathcal{W}(b^*)$. The following expectations are taken with respect to a uniformly chosen random pair of items from $P$. For $(i,j) \in P$, let %$Z_{(i,j)} :=(U_{i}^{\tau(i,j)} - U_{j}^{\tau(i,j)}) (U_{i}^{\tau(i,j)} - U_{j}^{\tau(i,j)})^T.$
%Let 
\begin{align*} Z_{(i,j)} &:=(U_{i}^{\tau(i,j)} - U_{j}^{\tau(i,j)}) (U_{i}^{\tau(i,j)} - U_{j}^{\tau(i,j)})^T
\\
\lambda &:= \lambda_{\min}( \mathbb{E} Z_{(i,j)}),\\ 
\eta &:= \sigma_{\max}(\mathbb{E}((Z_{(i,j)} - \mathbb{E}Z_{(i,j)})^2)),\\
\zeta &:= \max_{(k,\ell) \in P} \lambda_{\max}(\mathbb{E} Z_{(i,j)  } - Z_{ (k,\ell)}),
\end{align*}
%
where for a positive semidefinite matrix $X$, $\lambda_{\min}(X)$ and $\lambda_{\max}(X)$ are the smallest/largest eigenvalues of $X$, and where for any matrix $X$, $\sigma_{\max}(X)$ is the largest singular value of $X$. Let \begin{equation}
%\beta:=\max\left\{ \max_{(i,j) \in P} \| U_{i}^{\tau(i,j)} - U_{j}^{\tau(i,j)} \|_{\infty},1 \right\}. \label{eq:betadef}
\beta:=\max_{(i,j) \in P} \| U_{i}^{\tau(i,j)} - U_{j}^{\tau(i,j)} \|_{\infty}. \label{eq:betadef}
\end{equation}

% $$m \geq \max\left\{ O(\beta^2 d \log(d)), O((\eta + \lambda \zeta)log(d)/\lambda^2)\right\},$$ 
Let $\delta > 0$. If $\lambda>0$ and 
\begin{align*}
m \geq \max & \left\{C_1(\beta^2 d+\beta\sqrt{d}) \log(4d / \delta)\right., \\
& \left. C_2(\eta + \lambda \zeta)\frac{\log(2d / \delta)}{\lambda^2} \right\},    
\end{align*}
%$$m = \Omega\left(\max\left((\beta^2 d+\beta\sqrt{d}) \log(d) , (\eta + \lambda \zeta)\log(d)/\lambda^2 \right)\right),$$ 
%$$m = \Omega(\beta^2 d \log(d) + (\eta + \lambda \zeta)\log(d)/\lambda^2),$$
then with probability at least 
% Let \[m_1 := \frac{3B^2\log{(2d^2)}d + 4\sqrt{d}B \log{(2d^2)}}{6}\] and \[m_2 := \frac{8\log(d)(6\eta + \lambda R)}{3\lambda^2}. \] 
$1 - \delta$,
\begin{align*} 
\| w^* - \hat{w}\|_2 = O\left(\frac{\exp(b^*)}{\lambda}  \sqrt{\frac{(\beta^2 d+\beta\sqrt{d}) \log(4 d / \delta)}{m}}\right)
% & \frac{4(1 + \exp(b^*))^2}{\exp(b^*)\lambda}  \sqrt{\frac{3\beta^2\log{(2d^2)}d + 4\sqrt{d}\beta \log{(2d^2)}}{6m}}
\end{align*} 

where $C_1, C_2$ are constants given in the proof and the randomness is from the randomly chosen pairs and the outcomes of the pairwise comparisons.
\end{theorem}

 We utilize the proof technique of Theorem 4 in \cite{rankCentrality}, which proves a similar result for the standard BTL model of Equation \eqref{eq:BTL}, i.e. when $U=I_{n \times n}$, the $n \times n$ identity matrix, $d=n$, and $\tau(i,j) =[d]$ for all $(i,j) \in P$. We modify the proofs for arbitrary $U$ and $d$.  \todo{regular btl is actually not a special subcase} See Section \ref{appendix:sampleComplexityProof} in the Supplement for the proof. 
 
 We now discuss the terms that appear in Theorem \ref{thm:sampleComplexity}. First, the $d \log(d / \delta)$ terms are natural since we are estimating $d$ parameters. Second, estimating $w^*$ well essentially requires inverting the logistic function. When $b^*$ is large, we need to invert the logistic function for pairwise probabilities that are close to 0 and 1. This is precisely the challenging regime, since a small change in probabilities results in a large change in the estimate of $w^*$, and thus we expect to require many samples to estimate $w^*$ when $b^*$ is large. The exponential dependence on $b^*$ is standard for this type of analysis and arises from the Hessian of $\mathcal{L}_m$. Third, $\eta$ and $\zeta$ arise from a matrix concentration bound applied to the Hessian of $\mathcal{L}_m$. Fourth,  $\lambda$ arises from the minimum eigenvalue of the Hessian of $\mathcal{L}_m$ in a neighborhood of $w^*$, which controls the convexity of $\mathcal{L}_m$. This type of dependence also appears in other state of the art finite sample complexity analyses \cite{negahban2012unified}. In addition, to better understand the role of $\lambda$, we present the following proposition whose proof is in Section \ref{appendix:lambdaIdentifiable} in the Supplement. Proposition \ref{prop:lambdaIdentifiability} shows that the requirement $\lambda>0$ in Theorem \ref{thm:sampleComplexity} is fundamental, because we would otherwise be unable to bound the estimation error for the non-identifiable part of $w^*$, i.e., the projection of $w^*$ onto the orthogonal complement of $\text{span}\{ U_i^{\tau(i,j)} - U_j^{\tau(i,j)}: (i,j) \in P \} = \mathbb{R}^d$.
\begin{prop}
\label{prop:lambdaIdentifiability}
 $\lambda > 0$ if and only if the salient feature preference model is identifiable.
\end{prop}


Finally, if one assumes $\lambda, \eta, \zeta, \beta, \exp(b^*)$ are $O(1)$, then $\Omega(d \log (d / \delta))$ samples are enough to guarantee the error is $O(1)$. However, as we will show in the corollaries, these parameters are not always $O(1)$, increasing the complexity. We point out that the combination of the features $U$ and the selection function $\tau$ is what dictates the parameters of Theorem \ref{thm:sampleComplexity}. For the top-$t$ selection function in particular, we plot $\lambda, \zeta, \eta, b^*, \beta$, the number of samples required by Theorem \ref{thm:sampleComplexity}, and the bound on the estimation error as a function of intransitivity rates in the Supplement in Section \ref{appendix:parameterPlot}, to provide further insight into these parameters. Since we envision practical selection functions will be dependent on the features themselves, further analysis is a challenging but exciting subject of future work.

%Theorem \ref{thm:sampleComplexity} is only applicable when $\lambda > 0$, and Proposition \ref{prop:lambdaIdentifiability} says that this is a natural condition to require since if $\lambda = 0$, then the model is not identifiable, and we cannot estimate $w^*$. 

%The standard BTL model of Equation \eqref{eq:BTL} is not identifiable without assuming that the coordinates of $w^*$ sum to a constant, so Theorem \ref{thm:sampleComplexity} is not applicable in this case by Proposition \ref{prop:lambdaIdentifiability}.
% For the standard BTL model of Equation \eqref{eq:BTL}, $|\tau(i,j)| = d$ for any $(i,j) \in P$, $U = I_{n \times n}$ where $ I_{n \times n}$ is the $n \times n$ identity matrix, $d=n$, and $w^*$ contains the item utilities. However, Theorem \ref{thm:sampleComplexity} does not directly apply to the standard BTL model since it is not identifiable without additional assumptions on $w^*$, so Proposition \ref{prop:lambdaIdentifiability} implies $\lambda = 0$ in this case. \todo{We need to further assume that $\sum_{i=1}^n w^*_i = 0$ for identifiability since given $w^*$, adding the same constant to each entry of $w^*$ results in the same pairwise comparison probabilities. should I say anymore? i would like to say that you can think of $\lambda =  1/n$ and you get with $m \geq O(n \log(n))$ samples the error scales like $O(n^2 \log(n))$ }



For deterministic $U$, we now specialize our results to FBTL as well as to the case where a single feature is used in each comparison. The following corollaries provide insight into how a particular selection function $\tau$ impacts $\lambda$, $\eta$, and $\zeta$ and thus the sample complexity.

First, we consider FBTL. In this case, the selection function selects all the features in each pairwise comparison, so there cannot be intransitivities in the preference data. The following Corollary of Theorem \ref{thm:sampleComplexity} gives a simplified form for $\lambda$ and upper bounds $\zeta$ and $\eta$. The terms involving the conditioning of $UU^T$ are natural; since we make no assumption on $w^*$, if the feature vectors are concentrated in a lower dimensional subspace, estimation of $w^*$ will be more difficult. See Section \ref{appendix:specificSelectionFunctions} of the Supplement for the proof.
\begin{corollary}[Sample complexity for FBTL]
\label{coro:fullFeatures}
For the selection function $\tau$, suppose $|\tau(i,j)| = d$ for any $(i,j) \in P$. In other words, all the features are used in each pairwise comparison. Let $\nu := \max\{\max_{(i,j) \in P} \|U_i - U_j\|_2^2, 1\}$. Assume $n>d$. Without loss of generality, assume the columns of $U$ sum to zero: $\sum_{i = 1}^n U_i =0$. Let $\delta > 0$. Then,
\begin{align*}
\lambda &= \frac{n\lambda_{\min}(UU^T)}{\binom{n}{2}}, \\
\zeta &\leq \nu + \frac{n\lambda_{\max}(UU^T)}{\binom{n}{2}}, \text{ and } \\ 
\eta &\leq \frac{\nu n \lambda_{\max}(UU^T)}{\binom{n}{2}} + \frac{n^2 \lambda_{\max}(UU^T)^2}{\binom{n}{2}^2}.
\end{align*}

%$$\lambda = \frac{n\lambda_{\min}(UU^T)}{\binom{n}{2}},$$
%$$\zeta \leq \nu + \frac{n\lambda_{\max}(UU^T)}{\binom{n}{2}},$$ and 
%    $$\eta \leq \frac{\nu n \lambda_{\max}(UU^T)}{\binom{n}{2}} + \frac{n^2 \lambda_{\max}(UU^T)^2}{\binom{n}{2}^2}.$$ 
Hence, if 
\begin{align*} m \geq \max & \left\{ C_1(\beta^2 d+\beta\sqrt{d}) \log(4d / \delta) ,  \right. \\
 & \left. C_3 \log(2d / \delta) \nu n \bar\lambda \right\}
\end{align*}

where
$$\bar \lambda = \left( \frac{\lambda_{\max}(UU^T) + \lambda_{\max}(UU^T)^2 +  \lambda_{\min}(UU^T)}{\lambda_{\min}(UU^T)^2} \right)$$

%\begin{align} m  \geq \max\left\{&C_1(\beta^2 d+\beta\sqrt{d}) \log(d) , \right. \\ 
%&C_3 \log(d) \nu n \left. \left( \frac{\lambda_{\max}(UU^T) + \lambda_{\max}(UU^T)^2 }{\lambda_{\min}(UU^T)^2} \right.\right. \\
%&\hspace{2cm} + \left. \frac{1}{\lambda_{\min}(UU^T)} \right) \}
%\end{align}



% \begin{align*} 
% m  = \Omega\left( \frac{\nu \binom{n}{2} \lambda_{\max}(UU^T)}{n \lambda_{\min}(UU^T)^2} + \frac{\lambda_{\max}(UU^T)}{\lambda_{\min}(UU^T)} \right),
% \end{align*}
then with probability at least $1 - \delta$, \[\| w^* - \hat{w}\|_2 = O\left(\frac{\exp(b^*) n}{\lambda_{\min}(UU^T) } \sqrt{\frac{(\beta^2 d+\beta\sqrt{d}) \log( \frac{4d}{\delta})}{m}}\right)\]  
%where the randomness is from the randomly chosen pairs and the outcomes of the pairwise comparisons. 
where $C_1$ and $C_3$ are constants given in the proof.
\end{corollary}
\todo{what if U is sampled from Gaussian? you need to control the variance because if $U$ gets too big then $b^*$ gets too big}
\todo{add in $R$, and $C$, and if $U$ is drawn from a gaussian}

To the best of our knowledge, this is the first analysis of the sample complexity for the MLE of FBTL parameters. There are related results in \cite{fbtl, negahban2012unified, heckel2019active, shah2017simple} to which our bound compares favorably, and we discuss this in Section \ref{sec:boundcompare} of the Supplement.


Second, suppose the selection function is very aggressive and selects only one coordinate for each pair, i.e. $|\tau(i,j)|=1$ for all $(i,j) \in P$. For instance, the top-$1$ selection function has this property. This type of selection function can cause intransitivities in the preference data as we show in the synthetic experiments of Section \ref{sec:syntheticExperiments}. 
%The following corollary of Theorem \ref{thm:sampleComplexity} specializes the sample complexity results to this case by giving bounds on $\lambda, \eta,$ and $\zeta$.

\begin{corollary}
\label{coro:MaxCoordCoro}
Assume that for any $(i,j) \in P$, $|\tau(i,j)| = 1$. Partition $P = \sqcup_{k=1}^d P_k$ into $d$ sets where $(i,j) \in P_k$ if $\tau(i, j) = \{k\}$ for $k \in [d]$. Let $\beta$ be defined as in Theorem \ref{thm:sampleComplexity} and \[ \epsilon:= \min_{(i,j) \in P} \|U_i^{\tau(i,j)} - U_j^{\tau(i,j)}\|_{\infty}.\] Let $\delta > 0$.  Then
\begin{align*}
\lambda &\geq \frac{\epsilon^2}{ \binom{n}{2}}  \min_{k \in[d]} |P_k|,  \\
\zeta &\leq  \beta^2 + \frac{\beta^2}{ \binom{n}{2}} \max_{k \in [d]} |P_k|, \text{ and } \\
\eta &\leq \frac{\beta^4}{ \binom{n}{2}} \max_{k \in [d]} \left( |P_k| + \frac{|P_k|^2}{\binom{n}{2}} \right).
\end{align*}

% \[\lambda \geq \frac{\epsilon^2}{ \binom{n}{2}}  \min_{k \in[d]} |P_k|,\]
%    \[\zeta \leq  \beta^2 + \frac{\beta^2}{ \binom{n}{2}} \max_{k \in [d]} |P_k|,\] and
%    \[ \eta \leq \frac{\beta^4}{ \binom{n}{2}} \max_{k \in [d]} \left( |P_k| + \frac{|P_k|^2}{\binom{n}{2}} \right).\]
Hence, if 


% \begin{align*} 
% m  = \Omega\left( \beta^2 d \log(d) + \frac{\log{(d)} \beta^4  \max_{k \in [d]} \binom{n}{2} |P_k|}{ \epsilon^4 \min_{k \in [d]} |P_k|^2}\right),
% \end{align*}

$$m \geq \max\left\{C_1(\beta^2 d+\beta\sqrt{d}) \log(4d / \delta) ,  C_4(Q_1 + Q_2)  \right\},$$ 

where 
\begin{align*}
Q_1 &= \left(\frac{ \beta^4}{\epsilon^4}\right)\frac{\binom{n}{2} \max_{k \in [d]} |P_k| + \max_{k \in [d]} |P_k|^2}{\min_{k \in [d]} |P_k|^2}, \\
Q_2 &= \left(\frac{\beta^2}{\epsilon^2}\right)\frac{\binom{n}{2}  + \max_{k \in [d]} |P_k|}{\min_{k \in [d]} |P_k|},    
\end{align*}

%$$P_1 = \left(\frac{ \beta^4}{\epsilon^4}\right)\frac{\binom{n}{2} \max_{k \in [d]} |P_k| + \max_{k \in [d]} |P_k|^2}{\min_{k \in [d]} |P_k|^2}$$ and $$P_2 = \left(\frac{\beta^2}{\epsilon^2}\right)\frac{\binom{n}{2}  + \max_{k \in [d]} |P_k|}{\min_{k \in [d]} |P_k|},$$

then with probability at least $1 - \delta$, \[\| w^* - \hat{w}\|_2 = O\left(\frac{\exp(b^*) \binom{n}{2}}{ \epsilon^2 \underset{{k \in[d]}}{\min} |P_k| } \sqrt{\frac{(\beta^2 d+\beta\sqrt{d}) \log(\frac{4d}{\delta})}{m}}\right)\] 
where $C_1$ and $C_4$ are constants given in the proof.
%where the randomness is from the randomly chosen pairs and the outcomes of the pairwise comparisons. 

% let \[m_3 := \frac{ 8 \log(d) B^4 \max_{k \in [d]} \left( \binom{n}{2} |P_k| + |P_k|^2 \right)}{3 \epsilon^4 \min_{k \in[d]} |P_k|^2},\] \[m_4 := \frac{8 \log(d) B^2 \left(\binom{n}{2} + \max_{k \in [d]} |P_k| \right) }{3 \epsilon^2 \min_{k \in[d]} |P_k| }\].

% Hence, let \[m_3 := \frac{ 8 \log(d) B^4 \max_{k \in [d]} \left( \binom{n}{2} |P_k| + |P_k|^2 \right)}{3 \epsilon^4 \min_{k \in[d]} |P_k|^2},\] \[m_4 := \frac{8 \log(d) B^2 \left(\binom{n}{2} + \max_{k \in [d]} |P_k| \right) }{3 \epsilon^2 \min_{k \in[d]} |P_k| }\] and \[\beta :=  \frac{4(1 + \exp(b^*))^2 \binom{n}{2}}{\exp(b^*) \epsilon^2 \min_{k \in[d]} |P_k| }.\] If $m \geq \max\{m_1, m_3+m_4 \}$ where $m_1$ is defined in Theorem \ref{thm:sampleComplexity}, then with probability at least $1 - \frac{2}{d}$, \[\| w^* - \hat{w}\|_2 \leq \beta \sqrt{\frac{3B^2\log{(2d^2)}d + 4\sqrt{d}B \log{(2d^2)}}{6m}},\]  where the randomness is from the randomly chosen pairs and the outcomes of the pairwise comparisons.
\end{corollary}

 There are two main implications of Corollary \ref{coro:MaxCoordCoro} if we consider $\beta$ and $\epsilon$ constant. First, suppose there is a coordinate $k \in [d]$ such that $|P_k| := |\{(i,j) \in P: \tau(i,j)=k\}|$ is small. Intuitively it will take many samples to estimate $w^*$ well, since the chance of sampling a pairwise comparison that uses the $k$-th coordinate of $w^*$ is $|P_k| / \binom{n}{2}$. Corollary \ref{coro:MaxCoordCoro} formalizes this intuition. In particular, $\lambda=O(|P_k| / \binom{n}{2} )$, and since $\lambda$ comes into the bounds of Theorem \ref{thm:sampleComplexity} in the denominator of both the lower bound on samples and the upper bound on error, a small $\lambda$ makes estimation more difficult. %so the number of samples required and upper bound on the estimation error is large since $\lambda$ appears in the denominator for both the number of samples required and upper bound on the estimation error. %Hence, by Theorem \ref{thm:sampleComplexity}, many more samples are required to control the estimation error of $w^*$ compared to. 
 
 
Second, on the other hand, if $\epsilon$ is fixed, the maximum lower bound on $\lambda$ given by Corollary \ref{coro:MaxCoordCoro} is $ \max \min_{i \in [d]} |P_i| = \binom{n}{2} / d $ where the maximum is with respect to any partition of $P$. In this case, $|P_i| \approx |P_j|$ for all $i,j \in [d]$, so the chance of sampling a pairwise comparison that uses any coordinate is approximately equal. Therefore, $\lambda, \eta, \zeta = O(1/d)$, and by tightening a bound used in the proof of Theorem \ref{thm:sampleComplexity},  $\Omega(d^2\log(d / \delta))$ samples ensures the estimation error is $O(1)$. See Section \ref{sec:coroBoundTighten} in the Supplement for an explanation.
 %In this case, the sample complexity is independent of the number of items, which makes sense since adding additional items should not make learning the $d$ parameters of the judgment vector more difficult. \laura{what if number of items is very small?} \amanda{might not be identifiable} \todo{should i keep $B$ arbitrary because in this case, $B = 1/d$? also does this mean its tight by number of samples}
% However, by viewing the selection function $\tau$ as random, the analysis of  
% $\mathbb{E}_{\tau} (\lambda)$ where the expectation is with respect to the randomness of $\tau$ is manageable since we are essentially dealing with full features as in Theorem \ref{thm:fullFeatures}. Because $\lambda$ shows up in the denominator of $B_m$ and in $m_2$ in Theorem \ref{thm:sampleComplexity}, we seek to lower bound $\lambda$ for a deterministic $U$, which is what the following theorem does. \todo{should we try to make a connection between this selection function and picking based on variance because under a gaussian it shouldnt favor any one coordinate. you are basically including each coordinate with probability p}
% \begin{theorem}
% \label{thm:randomSelection}
% Let $U \in \R^{d \times n}$, $w^* \in \R^d$, $\tau$, and $S_m$ be defined as in the beginning of this section except where the selection function $\tau$ is random: before the samples $S_m$ are collected, for each $(i,j) \in P$, $ k \in \tau(i,j)$ for $k \in [d]$ with probability $p$ independently from other coordinates and other pairs of items. Without loss of generality, assume the columns of $U$ sum to zero: $\sum_{i = 1}^n U_i =0$. Let \[D = \mathrm{diag}\left(\sum_{(i,j) \in P} (U_i-U_j) \circ (U_i-U_j) \right),\] then 
% \begin{align}
%     \mathbb{E}_{\tau} (\lambda) &:=  \mathbb{E}_{\tau} (\lambda_{\min}(\mathbb{E}((U_{i} - U_{j}) (U_{i} - U_{j})^T))) \\  
%     &\geq \frac{n p}{\binom{n}{2}} \left(\lambda_{\min}\left(pUU^T + \frac{(1-p)}{n} D \right)\right)
% \end{align}
% where $X \circ Y$ is the Hadamard product of two matrices $X$ and $Y$, $\mathrm{diag}(x)$ is the diagonal matrix whose $(i,i)$-th entry is the $i$-th entry of the vector $x$, and the outer expectation is taken with respect to the random selection function $\tau$ and the inner expectation is with respect to a uniformly at random chosen pair of items. \todo{argue for why looking at the expectation is good}
% \todo{add in $R$, and $C$, and if $U$ is drawn from a Gaussian} 
% \end{theorem}

% Notice that when $p=1$ in Theorem \ref{thm:randomSelection}, i.e. the selection function always outputs each coordinate, we recover Theorem \ref{thm:fullFeatures}. 



% In particular, under a particular distribution from which $U$ is draw, we demonstrate how as the size of $|\tau(i,j)|$ decreases for $(i,j) \in P$, $\lambda$ decreases. This empirical result along with Theorem \ref{thm:sampleComplexity} suggests that more intransitives makes learning the judgement vector harder.

\todo{
\begin{itemize}
\item need to talk about how number of items affects things (maybe it does not if d =1, then lambda i guess is like constant? + add plots for this) and just interpret all these results
\end{itemize}
}

% An extensive investigation of how a particular selection function $\tau$ impacts $\lambda$ is of interest for future work.
% As a sanity check, if there is a feature $k$ such that $ k \notin \tau(i,j)$ for any $i,j \in [n]$, then it is impossible to learn $w_k$, and in this case, $\lambda = 0$, so Theorem \ref{thm:sampleComplexity} does not apply. 
%See Section \ref{appendix:lambdaPositive} in the Supplement for discussion about when $\lambda >0.$ In our synthetic experiments, we observe $\lambda > 0$.
%In Section \ref{appendix:lambdaPositive} in the Supplement, we provide two selection functions such that $\lambda >0$. In particular, when the selection function evaluates to a single feature, we show $\lambda>0$, and when the selection function returns every feature, we show $\lambda = \lambda_{\min}(UU^T)$.

Ultimately, we seek to estimate the underlying ranking of the items. The following corollary of Theorem \ref{thm:sampleComplexity} says that by controlling the estimation error of $w^*$, the underlying ranking can be estimated approximately. %To the best of our knowledge, Corollary \ref{coro:rankingComplexity} is the first sample complexity result for learning a ranking on a set of items where the observed pairwise preferences violate transitivity. 
%The work in \cite{niranjan2017inductive} has a similar type of result but they assume that the pairwise preferences are transitive. 
The sample complexity depends inversely on the square of the differences of full feature item utilities. Intuitively, if the absolute difference between the utilities of two items is small, then many samples are required in order to rank these items correctly relative to each other. 
See Section \ref{appendix:coroRankingProof} in the Supplement for the proof.
% \begin{corollary}[Sample complexity of learning the ranking exactly]
% \label{coro:rankingComplexity}
% Assume the set-up of Theorem \ref{thm:sampleComplexity}. Let $\alpha = \min_{(i,j) \in P} | \langle w^*, U_i - U_j \rangle|$ be the smallest difference in full-feature utilities and $M = \max_{i \in [n]} \|U_i\|_2$. Let $\gamma^*: [n] \rightarrow [n]$ be the ranking obtained from $w^*$ by sorting the items by their full-feature utilities $\langle w^*, U_i\rangle$ where $\gamma(i)$ is the position of item $i$ in the ranking. Define $\hat{\gamma}$ similarly but for the estimated ranking obtained from the MLE estimate $\hat{w}$. If \[m \geq \max\left\{\frac{64 M^2(1 + \exp(b^*))^4}{\alpha^2 \exp(b^*)^2\lambda^2}, \frac{d}{\left(\frac{ 3 }{2B\log{{2d^2}}  } - 3 d B \right)^2}, \frac{8\log(d)(6C + 2\lambda D_{U, \tau})}{3\lambda^2} \right\},\] then with probability $1 - \frac{2}{d}$, $\gamma^* = \hat{\gamma}.$

% \begin{corollary}[Sample complexity of estimating the ranking]
% \label{coro:rankingComplexity}
% Assume the set-up of Theorem \ref{thm:sampleComplexity}. Pick $k \in [\binom{n}{2}]$. Let $\alpha_k$ be the $k$-th smallest number in $\{ |\langle w^*, U_i - U_j \rangle|: (i,j) \in P \}$. Let $M := \max_{i \in [n]} \|U_i\|_2$. Let $\gamma^*: [n] \rightarrow [n]$ be the ranking obtained from $w^*$ by sorting the items by their full-feature utilities $\langle w^*, U_i\rangle$ where $\gamma^*(i)$ is the position of item $i$ in the ranking. Define $\hat{\gamma}$ similarly but for the estimated ranking obtained from the MLE estimate $\hat{w}$. Let $m_1$ and $m_2$ be defined as in Theorem \ref{thm:sampleComplexity}. Let \[m_3 := \frac{64 M^2 (1 + e^{b^*})^4 B \log{(2d^2)} (3Bd + 4\sqrt{d})}{6\alpha_k^2 e^{2b^*}\lambda^2}.\] If $m \geq \{m_1, m_2, m_3\}$, then with probability $1 - \frac{2}{d}$, \[K(\gamma^*,\hat{\gamma}) \leq k-1,\] where $K(\gamma^*, \hat{\gamma}) = |\{(i,j) \in P: (\gamma^*(i) - \gamma^*(j))(\hat{\gamma}(i) - \hat{\gamma}(j)) >0\}|$ is the Kendall tau distance between two rankings.
% \end{corollary}
\begin{corollary}[Sample complexity of estimating the ranking]
\label{coro:rankingComplexity}
Assume the set-up of Theorem \ref{thm:sampleComplexity}. Pick $k \in [\binom{n}{2}]$. Let $\alpha_k$ be the $k$-th smallest number in $\{ |\langle w^*, U_i - U_j \rangle|: (i,j) \in P \}$. Let $M := \max_{i \in [n]} \|U_i\|_2$. Let $\gamma^*: [n] \rightarrow [n]$ be the ranking obtained from $w^*$ by sorting the items by their full-feature utilities $\langle w^*, U_i\rangle$ where $\gamma^*(i)$ is the position of item $i$ in the ranking. Define $\hat{\gamma}$ similarly but for the estimated ranking obtained from the MLE estimate $\hat{w}$. Let $\delta > 0$. If 
\begin{align*}
m \geq \max & \left\{  C_1(\beta^2 d+\beta\sqrt{d}) \log(4d / \delta) ,\right. \\
& \left. C_2(\eta + \lambda \zeta)\frac{\log(2d / \delta)}{\lambda^2},\right. \\
& \left. \frac{C_5  M^2 e^{2b^*} (\beta^2 d+\beta\sqrt{d}) \log(4d / \delta)}{\alpha_k^2 \lambda^2} \right\},
\end{align*}
then with probability $1 - \delta$, \[K(\gamma^*,\hat{\gamma}) \leq k-1,\] where $K(\gamma^*, \hat{\gamma}) = |\{(i,j) \in P: (\gamma^*(i) - \gamma^*(j))(\hat{\gamma}(i) - \hat{\gamma}(j)) <0\}|$ is the Kendall tau distance between two rankings and $C_1$, $C_2$, and $C_5$ are constants given in the proof. 
\end{corollary}

%for every $(i,j) \in P$, $\left(\langle \hat{w}, U_i \rangle - \langle \hat{w}, U_j \rangle \right) \left(\langle w^*, U_i \rangle - \langle w^*, U_j \rangle \right) >0$. In other words, 
%Let $\gamma^*: [n] \rightarrow [n]$ where $t_i^* \in [n]$ and $\hat{\gamma} = (\hat{t}_1, \dots, \hat{t}_n)$ where $\hat{t}_i \in [n]$ be the rankings of the items obtained by sorting the items by their utilities when all features are utilized: $\langle w^*, U_i \rangle$ and $\langle \hat{w}, U_i \rangle$, respectively.  the ranking $\gamma^* = \hat{\gamma}.$
% \end{corollary}


% One of the main assumptions in Theorem \ref{thm:sampleComplexity} is that $\lambda >0$, so we now provide a scenario on the selection function where $\lambda >0$.
% \begin{corollary}
% \label{coro:maxCoord}
% Assume the set-up of Theorem \ref{thm:sampleComplexity}. WLOG, assume that the sum of the columns of $U$ is 0: $\sum_{i=1}^n U_i = 0$. For any $i,j \in [n]$, if $|\tau(i,j)|=1$, then $\lambda > ??$.
% \end{corollary}
% \todo{move to appendix}



% \begin{theorem}
% Talk about specific scenarios where the previous theorem can or cannot be applied.
% Ideas:
% \begin{itemize}
%     \item BTL with features: $\lambda = \lambda_{\min} UU^T$ assuming $U$ has full row rank and sum of the columns of $U$ are 0. (can do this!)
%     \item If there is a scenario where only one feature is used per pairwise comparison, then we can maybe say something. Or more generally, if there is a scenario where the intersection of any two $\tau(i,j$ is either empty or equal.
%     \item if features used between pairs of items are chosen randomly instead of the features that stick out the most.
%     \item $\lambda = 0$ when one feature is never used since there is no way to recover $w^*$
% \end{itemize}
% \end{theorem}
% \begin{proof}
% First, \[(U_{i_\ell}^{\tau_{t}(T_\ell)} - U_{j_\ell}^{\tau_{t}(T_\ell)}) (U_{i_\ell}^{\tau_{t}(T_\ell)} - U_{j_\ell}^{\tau_{t}(T_\ell)})^T = I_{\tau_{t}(T_\ell)}U x_{(i_\ell, j_\ell)} x_{(i_\ell, j_\ell)}^T U^T I_{\tau_{t}(T_\ell)}\] 
% where $I_{\tau_{t}(T_\ell)} \in \mathbb{R}^{d \times d}$ such that $(I_{\tau_{t}(T_\ell)})_{ii} = 1$ if $i \in \tau_{t}(T_\ell)$ and 0 otherwise and where $x_{(i_\ell, j_\ell)} = (e_i - e_j)(e_i - e_j)^T$ where $e_i$ is the $i$-th standard basis vector. 

% Let \todo{maybe change the $\ell$ notation in the expectation}
% \begin{align}
%     X_\ell = \frac{1}{m} I_{\tau_{t}(T_\ell)}U x_{(i_\ell, j_\ell)} x_{(i_\ell, j_\ell)}^T U^T I_{\tau_{t}(T_\ell)} - \frac{1}{m} \mathbb{E}(I_{\tau_{t}(T_\ell)}U x_{(i_\ell, j_\ell)} x_{(i_\ell, j_\ell)}^T  U^T I_{\tau_{t}(T_\ell)}) 
% \end{align}
% where the expectation is with respect to the random pair drawn.

% Let $P =\{(i,j) \in [n] \times [n]: i<j\}$ be the set of all the pairs of items. Let $K = \{\tau(i,j): (i,j) \in P\}$ and $T_k \subseteq P$ such that $(a,b), (i,j) \in T_k$ if $\tau(i,j) = \tau(\{a,b\}) = k$. 

% Let \todo{maybe change the $\ell$ notation in the expectation}
% \begin{align}
%     X_\ell = \frac{1}{m} I_{\tau_{t}(T_\ell)}U x_{(i_\ell, j_\ell)} x_{(i_\ell, j_\ell)}^T U^T I_{\tau_{t}(T_\ell)} - \frac{1}{m} \mathbb{E}(I_{\tau_{t}(T_\ell)}U x_{(i_\ell, j_\ell)} x_{(i_\ell, j_\ell)}^T  U^T I_{\tau_{t}(T_\ell)}) 
% \end{align}
% where the expectation is with respect to the random pair drawn.


% Let $P =\{(i,j) \in [n] \times [n]: i<j\}$ be the set of all the pairs of items. Let $K = \{\tau(i,j): (i,j) \in P\}$ and $T_k \subseteq P$ such that $(a,b), (i,j) \in T_k$ if $\tau(i,j) = \tau(\{a,b\}) = k$. Then $\{T_k\}_{k \in K}$ is a partition of $P$. Then
% \begin{align}
%     \mathbb{E}(I_{\tau_{t}(T_\ell)}U x_{(i_\ell, j_\ell)} x_{(i_\ell, j_\ell)}^T U^T I_{\tau_{t}(T_\ell)}) &= \frac{1}{\binom{n}{2}} \sum_{k \in K} I_{k}U \left( \sum_{(i,j) \in T_k} x_{(i,j)} x_{(i,j)}^T \right) (I_{k} U)^T \\
%     &= \frac{1}{\binom{n}{2}} \sum_{k \in K} I_{k}U \left( \sum_{(i,j) \in T_k} x_{(i,j)} x_{(i,j)}^T \right) (I_{k} U)^T \\
%     &= \frac{1}{\binom{n}{2}} \sum_{k \in K} I_{k}U \left( N_{T_k} - \mathbbm{1}_{T_k} \mathbbm{1}_{T_k}^T \right) (I_{k} U)^T   \text{ by Lemma \ref{lem:expectationOfXX} in the Supplement }
% \end{align}
% where $N_k \in \mathbb{R}^{n \times n}$ such that $(N_k)_{ii} =  |\{j: (i,j) \in T_k \}| + \mathbbm{1}_{\{ \exists j \in [n]: (i,j) \in T_k\}}$ and $(N_{k})_{i,j} = 0$ if $ i\neq j$ and where $\mathbbm{1}_{T_k} \in \mathbb{R}^n$ such that $(\mathbbm{1}_{T_k})_i = 1$ if there exists $j \in [n]$ such that $(i,j) \in T_k$.

% Continuing,
% \begin{align}
%     & \frac{1}{\binom{n}{2}} \sum_{k \in K} I_{k}U \left( N_{T_k} - \mathbbm{1}_{T_k} \mathbbm{1}_{T_k}^T \right) (I_{k} U)^T \\
%     & = \frac{1}{\binom{n}{2}} \left(\sum_{k \in K}  I_{k}U  N_{T_k} (I_{k} U)^T   \right) - \frac{1}{\binom{n}{2}}\left( \sum_{k \in K} I_{k} U \mathbbm{1}_{T_k} \mathbbm{1}_{T_k}^T  (I_{k} U)^T  \right) \\
%     & = \frac{1}{\binom{n}{2}} \left(\sum_{k \in K}  \left(I_{k}U \sqrt{N_{T_k}}\right)   \left(I_{k} U \sqrt{N_{T_k}})^T   \right) \right) - \frac{1}{\binom{n}{2}} \left( \sum_{k \in K} I_{k} U \mathbbm{1}_{T_k} \mathbbm{1}_{T_k}^T  (I_{k} U)^T  \right).
% \end{align}
% \end{proof}

% \subsection{Interpolation between pairwise comparisons and $k$-wise comparisons}
% \begin{theorem}
% Assume the entries of $U \in \mathbb{R}^{d \times n}$ are drawn independently from a distribution $f$ where the variance of $f$ is $\gamma^2 < \infty$. Let the threshold function be the independent sample variance threshold with threshold $\gamma^2 + \epsilon$. Then as $n,k \rightarrow \infty$, let $Uniform(k)$ be the uniform distribution on all $k-tuples$
% \begin{align}
%     \mathbb{E}_{U \sim f, T \sim Uniform(k)}(|\tau(T)|) \rightarrow d.
% \end{align}
% \end{theorem}
% In this section, let $U_{i,j} \sim N(0,1)$ be iid. 

% \begin{lemma}
% Let $\{X_i\}$ be a set of symmetric iid random variables. Then the set of pairwise differences $\{|X_i - X_j| \}_{(i,j)}$ are pairwise independent.
% \end{lemma}
% \begin{proof}
% \begin{align}
%     & \mathbb{P}(|X_i - X_j| = a | |X_i - X_k| = b) \\ 
%     & =\mathbb{P}(|X_i - X_j| = a | |X_i - X_k| = b| X_i \geq X_k) \mathbb{P}(X_i \geq X_k) + \mathbb{P}(|X_i - X_j| = a | |X_i - X_k| = b| X_k \geq X_i) \mathbb{P}(X_k \geq X_i) \\ 
%     &= \frac{1}{2}(\mathbb{P}(X_j - X_i = a | |X_i - X_k| = b| X_i \geq X_k) + \mathbb{P}(|X_i - X_j| = a | X_k - X_i = b| X_k \geq X_i))
% \end{align}
% \end{proof}
% \begin{lemma}
% Let $U_{i,j} \sim N(0,1)$ be iid. If $\tau = \mathbb{E} (h_{1, w^*}) + \epsilon$ for appropriate $\epsilon$, then $\mathbb{P}( | \Omega_{T_k} | > | \Omega_{T_{\ell}} | ) > .5$ where $T_j$ is a set of items of size $j$ and the probability is over the randomness of $U$.
% \end{lemma}

% \todo{Add an explicit small example?}

==> main/zappos.tex <==
\paragraph{\texttt{UT Zappos50k}}
The \texttt{UT Zappos50K} data set consists of pairwise comparisons on images of shoes and 960 extracted vision features for each shoe \cite{finegrained, semjitter}. Given images of two shoes and an attribute from $\{$``open,'' ``pointy,'' ``sporty,'' ``comfort''$\}$, respondents picked which shoe exhibited the attribute more. The data consists of easier, coarse questions, i.e. based on comfort, pick between a slipper or high-heel, and harder, fine grained questions i.e. based on comfort, pick between two slippers. 
%There were two sets of experiments: one with coarser questions, i.e. based on comfort, pick between a slipper or high-heel, and one with fine-grained questions, i.e. based on comfort, pick between two slippers. 

We now consider predicting pairwise comparisons instead of estimating a ranking since there is no ranking data available. We train four models, one for each attribute. See Table \ref{table:zappos} for the average pairwise comparison accuracy over ten train (70\%),  validation (15\%), and test splits (15\%) of the data. The pairwise comparison accuracy is defined as the percentage of items $(i,j)$ where $i$ beats $j$ a majority of the time and the model estimates the probability that $i$ beats $j$ exceeds $50\%$. 

In this case, the MLE of the FBTL model and the salient feature preference model under the top $t$ selection function perform similarly. Nevertheless, while the FBTL model utilizes all 990 features, the best $t$'s on each validation set and split of the data do not use all features, so our model is different from yet competitive to FBTL. See Table \ref{table:zapposT} in the Supplement. This suggests that the salient feature preference model under the top-$t$ selection function for relatively small $t$ is still a reasonable model for real data.
%Furthermore, because the data is high dimensional and the features do not correspond to  

==> synthetic_experiments_old.tex <==
We highlight the differences between the salient feature preference model and the FBTL model, investigate violations of rational choice arising from the salient feature preference model, and illustrate Theorem \ref{thm:sampleComplexity}. Given the very reasonable simulation setup we use, these experiments suggest that the salient feature preference model may sometimes be better suited to real data than the FBTL model. We present results on the top-$t$ selection function. 
%See Section \ref{appendix:figs} of the Supplement for the corresponding experiments for the RISV selection function.

First, under the salient feature preference model, we investigate the affect of the threshold of the RASV selection function on learning $w^*$ and the underlying ranking. We set $n = 200$, $d = 20$, $m = 10,000$, and sample columns of $U \in \mathbb{R}^{d \times n}$ from a Gaussian mixture model $\sum_{i = 1}^4 \frac{1}{4} \mathcal{N}(\mu_i,I)$ where $\mu_i \sim N(0, \sqrt{3}I)$, and $w \in \mathbb{R}^d \sim \mathcal{N}(0,I)$ and normalized to have unit norm. For a fixed $U$ and $w$, 10,000 pairwise comparisons are sampled from the salient feature preference model of Equation \eqref{eq:thresholdBTL} with the RASV selection function of Equation \eqref{eq:AVT} with threshold $t \in \{.05, .1, \dots, .95, 1\}$. This procedure is repeated 10 times with a new $U$ and $w$. 


The first plot in Figure \ref{fig:syntheticExperiments} shows the average estimation error of $w^*$ on the logarithmic scale, i.e. $\frac{1}{10} \sum_{i=1}^{10} \log_{10}(\|w^* - \hat{w}_i\|_2 )$, and the standard deviation of the MLE of the salient feature preference model with the RASV selection function and the BTL model. The second plot in Figure \ref{fig:syntheticExperiments} shows the Kendall tau correlation between the true ranking (obtained by ranking the items according to $\langle U_i, w^* \rangle$) and the estimated ranking (according to $\langle U_i, \hat{w} \rangle$). The Kendall tau correlation between two rankings $\sigma, \rho: [n] \rightarrow [n]$ on $n$ items, where $\sigma(i)$ is the position of item $i$ in the ranking, is defined as
\begin{align}
    \text{KT}(\sigma, \rho) = \frac{\sum_{(i,j) \in P} \mathbbm{1}_{\{(\sigma(i) - \sigma(j))(\rho(i) - \rho(j))>0\}} - \sum_{(i,j) \in P} \mathbbm{1}_{\{(\sigma(i) - \sigma(j))(\rho(i) - \rho(j))\leq 0\}} }{\binom{n}{2}}.
\end{align}
$\mathrm{KT}(\sigma,\rho) = 1$ when $\sigma = \rho$, and $\mathrm{KT}(\sigma,\rho) = 0$ means $\sigma$ and $\rho$ agree on the same number of pairwise comparisons as they disagree on. 
%The ranking obtained by the BTL MLE without features estimates the ranking more poorly than the BTL with features MLE since it is not utilizing the item features. 
%Although Theorem \ref{thm:sampleComplexity} does not imply that the Kendall tau correlation of the resulting ranking obtained by the MLE of $w^*$ and the true ranking will converge to 1, we see that the MLE produces a ranking that is close to the true ranking. \todo{take this sentence out?}
For every threshold $t < 1$, there is a gap between the estimation error of $w^*$ (and the Kendall tau correlation) under the MLE of the salient feature preference model and the MLE of the BTL model, illustrating that the salient feature preference model is quantitatively different than the BTL model though we remark that this gap is expected since the synthetic preference data is generated with respect to the RASV model, not the BTL model. Furthermore, we expect that as the threshold increases, the gap between the two models improves since the RASV model -- which is how the data is generated -- becomes more and more like the BTL model since more and more features will be used in each context-dependent comparison.

\begin{figure}%
    \centering
    \includegraphics[width=14cm]{figs/synthetic_experiment_figs/w_error_KT_RASV.pdf}
    \caption{First two figures: For 10,000 samples from the salient feature preference model with the RASV selection function, there is a significant gap between the MLE of the BTL model and the salient feature preference model on the estimation error of $w^*$ and the Kendall tau correlation of the estimated ranking with the true ranking. Last figure: Illustration of Theorem \ref{thm:sampleComplexity} for the salient feature preference model under the RASV selection function with threshold $t = .4$.}
    \label{fig:syntheticExperiments}%
\end{figure}

%Third figure: systematic intransitives arise under the same sampling model of the first two plots.

% \begin{figure}%
%     \centering
%     \subfloat{{\includegraphics[width=5cm]{synthetic_experiment_figs/w_error_threshold_sweep_indp.pdf}
%     }}%
%     \subfloat{{\includegraphics[width=5cm]{synthetic_experiment_figs/w_error_threshold_sweep_indp.pdf} }}%
%     \caption{2 Figures side by side}%
%     \label{fig:example}%
%     \subfloat{{\includegraphics[width=5cm]{synthetic_experiment_figs/w_error_threshold_sweep_indp.pdf}
%     }}%
%     \subfloat{{\includegraphics[width=5cm]{synthetic_experiment_figs/w_error_threshold_sweep_indp.pdf} }}%
%     \caption{2 Figures side by side}%
%     \label{fig:example}%
% \end{figure}

%\includegraphics[width=7cm]{synthetic_experiment_figs/w_error_threshold_sweep_additive.pdf}

% \begin{figure}%
%     \centering
%     \subfloat[test]{{\includegraphics[width=8cm]{synthetic_experiment_figs/w_KT_additive.pdf} }}%
%     \qquad
%     \subfloat[label 2]{{\includegraphics[width=5cm]{synthetic_experiment_figs/w_error_threshold_sweep_additive.pdf} }}%
%     \caption{2 Figures side by side}%
%     \label{fig:example}%
% \end{figure}
%As the threshold increases, the estimation error of $w^*$ decreases and similarly the Kendall tau correlation increases. 
%The MLE of the BTL model struggles much more with intransitivity and pairwise comparisons that are inconsistent with the underlying ranking. 

%and while our salient feature preference model can handle these issues, it will require more samples to learn $w^*$ well the more these issues are present. When the threshold is equal to 1, both the BTL with features model and our salient feature preference model are equivalent since all the features are utilized in the utilities. \todo{LKB took this out because of course we can learn w* when it follows our likelihood model and we have enough data. The point is more that BTL does not still do fine.}
 \todo{should i comment about why the blue line in the left plot is not perfectly monotonic?}
\todo{should i comment about how the red line on the left side plot has small variance, but large variance on the right handside? I guess this says that the BTL MLE estimator produces utilities that are very close.}

% Our salient feature preference model results in pairwise comparisons that violate properties that pairwise comparisons drawn from a standard BTL model must satisfy. Since these properties likely dictate the difficulty of learning $w^*$, we plot these properties. We use all pairs and the exact pairwise probabilities instead of empirical. We depict the average and standard deviation over the 10 trials with the same 10 $U$ and $w$ from the previous experiment.

Second, the salient feature preference model produces preferences that systematically violate rational choice, which can explain why the MLE of the BTL model struggles to estimate $w^*$ since BTL fundamentally cannot model these violations. Let $P_{ij} = \mathbb{P}(i>j)$ and $T = \{ (i,j,k) \in [n]^3: P_{ij} \geq .5, P_{jk}\geq.5\}$, then $(i,j,k) \in T$ satisfies strong stochastic transitivity if $P_{ik}\geq \max\{P_{ij}, P_{jk} \}$, moderate stochastic transitivity if $P_{ik} \geq \min\{P_{ij}, P_{jk} \}$, and weak stochastic transitivity if $P_{ik} \geq .5$ \cite{cattelan2012models}. The first plot in Figure \ref{fig:propsRASV} shows the average ratio of the number of weak, moderate, strong stochastic transitivity violations to $|T|$ with the standard deviation from the the same ten $U$ and $w$ from the previous experiment where we use all of the exact pairwise probabilities given by the salient feature preference model under the RASV selection function. Furthermore, the salient feature preference model produces pairwise comparisons that are inconsistent with the underlying true ranking. Consider items $i,j$ such that $\langle U_{i} - U_{j}, w^* \rangle < 0$, meaning item $i$ is ranked lower than item $j$ in the ranking. This pair may be such that $\langle U_{i}^{\tau_{t}(i,j)} - U_{j}^{\tau_{t}(i,j)}, w^* \rangle >0$ meaning item $i$ beats item $j$ by at least 50\% when compared in isolation from the other items. See the second plot in Figure \ref{fig:propsRASV}, which shows what percentage of pairwise comparisons of all pairwise comparisons are inconsistent with the true ranking under the same set-up of the intransitivity results. Although a synthetic example, real data exhibits intransitivity and inconsistent pairs with the underlying ranking as shown in the real data experiments.

\begin{figure}%
    \centering
    \includegraphics[width=12cm]{figs/synthetic_experiment_figs/rational_violation_RASV.pdf}
    \caption{The salient feature preference model with the RASV selection function produces systematic intransitives and pairwise comparisons that are inconsistent with the underlying ranking.}
    \label{fig:propsRASV}
\end{figure}

% Second, 

% Third, Figure \ref{fig:syntheticExperiments} also shows the low noise violation rate which is the fraction of pairs for which the low noise condition does not hold. The low noise condition is a property of the underlying pairwise probabilities and is defined as the following implication: if for any pair of items $(i,j)$ $P_{ij} > .5$, then $\sum_{k} P_{ki} > \sum_{k} P_{kj}$. The low noise condition is a sufficient condition for the MLE of the BTL without features model to produce a ranking that minimizes the number of pairs that disagree with the underlying ranking \cite{rajkumar2016can}.

% Since the salient feature preference model only uses some features for each pairwise comparison, we consider how many features on average are used by each pairwise comparison. See Figure \ref{fig:syntheticExperiments}. Other than when the threshold is 1, no sampled pairwise comparison utilizes all the features in the resulting utilities, i.e. $\tau_t(\{i,j\}) \neq [d].$ As one might expect, in the regime where only a few features are used is where the most intransitives and inconsistencies with the underlying ranking arise.

% \begin{figure}%
%     \centering
%     \includegraphics[width=15cm]{synthetic_experiment_figs/props_additive.pdf}
%     \caption{The effect of varying the threshold of the salient feature preference model with the RASV selection function on properties of the pairwise comparisons. This model produces a significant number of intransitive preferences and also pairwise comparisons that disagree with the underlying ranking especially for small thresholds. }%
%     \label{fig:syntheticExperiments}%
% \end{figure}

 %model in certain scenarios especially since the sampling distribution, which is a mixture of Gaussians, for $U$ is reasonable.

Finally, we illustrate Theorem \ref{thm:sampleComplexity} under the salient feature preference model with the RASV selection function with threshold $t =.4$. $U$ and $w$ are sampled once from the same distribution as before. We sample $m$ pairwise comparisons for $m \in \{1000, 5000, 10000, 25000, 50000, 75000\}$, fit the MLEs, and repeat 5 times. The last plot in Figure \ref{fig:syntheticExperiments} shows the average estimation error of $w^*$ on the logarithmic scale with the standard deviation and also the theoretical bound of Theorem \ref{thm:sampleComplexity}. Since $U$ and $w$ are fixed, the bound is valid for the entire experiment. There is a gap between the observed error and the theoretical bound, though the error decreases at the same rate. Furthermore, the number of samples required by Theorem \ref{thm:sampleComplexity} is often on the order of $10^6$ for these experiments, much greater than what we observe is required. However, the error of the MLE of BTL does not improve with more samples, likely because of the intransitives and inconsistent pairs.

% \begin{figure}%
%     \centering
%     \includegraphics[width=7cm]{synthetic_experiment_figs/w_error_threshold_sweep_additive.pdf}
%     \caption{The affect of varying the threshold on properties of the pairwise comparisons under the RASVmodel.}%
%     \label{fig:thmIllustration}%
% \end{figure}


% \begin{figure}%
%     \centering
%     \subfloat{{\includegraphics[width=9cm]{synthetic_experiment_figs/w_error_threshold_sweep_additive.pdf} }}%
%     \qquad
%     \subfloat{{\includegraphics[width=9cm]{synthetic_experiment_figs/w_error_threshold_sweep_additive_zoom.pdf} }}%
%   \caption{The affect of varying the threshold on properties of the pairwise comparisons under the RASV model.}%
%     \label{fig:thmIllustration}%
% \end{figure}
 

% First, we consider the case when all the features are used in each pairwise comparison, i.e., the threshold function $\tau_t$ is constant and always evaluates to $[d]$ where $d$ is the dimension of the features of the items. Each entry of $U \in \mathbb{R}^{d \times n}$ and $w \in \mathbb{R}^d$ is drawn from $\mathcal{N}(0,1)$ then $w$ is normalized to have unit norm. For this fixed $U$ and $w$, we sample $x \in \{2000, 4000, 6000, 8000, 10000\}$ pairwise comparisons chosen independently and uniformly at random and then find the MLE $\hat{w}$ of $w$. For each choice of number of samples, we repeat this process 5 times by sampling new pairwise comparisons and then computing $\hat{w}$. We use $d = 10$ for the dimension of the features and $n = 200$ for the number of items.

% Figure \ref{fig:thresholdAllwError} shows the average over the 5 trials of the estimation error of $w^*$  on the logarithmic scale given by $\log(\|w^* - \hat{w}\|_2 )$ with the standard deviation of the 5 trials and also the theoretical bound given by Theorem \ref{thm:sampleComplexity}. Since $U$ and $w$ are fixed, this theoretical bound holds for each of the 5 trials. In this case, the BTL with features model and the salient feature preference model are identical. We also plot the Kendall tau correlation between the true ranking obtained by ranking the items by $\langle U_i, w^* \rangle$ and also the estimated ranking by ranking the items by $\langle U_i, \hat{w} \rangle$ where the Kendall tau correlation between two rankings $\sigma, \tau: [n] \rightarrow [n]$ on $n$ items is defined as
% \begin{align}
%     \text{KT}(\sigma, \tau) = \frac{\sum_{(i,j) \in P} \mathbbm{1}_{\{(\sigma(i) - \sigma(j))(\tau(i) - \tau(j))>0\}} - \sum_{(i,j) \in P} \mathbbm{1}_{\{(\sigma(i) - \sigma(j))(\tau(i) - \tau(j))\leq 0\}} }{{n \choose 2}}
% \end{align}
% where $\sigma(i)$ is the position of item $i$ in the ranking. The ranking obtained by the BTL MLE without features has a slower convergence to the true ranking, which makes sense since it is not utilizing feature information about the items.

% \begin{figure}%
%     \centering
%     \subfloat{{\includegraphics[width=8cm]{synthetic_experiment_figs/w_error_all.pdf} }}%
%     \qquad
%     \subfloat{{\includegraphics[width=8cm]{synthetic_experiment_figs/kt_all.pdf} }}%
%     \caption{All features are used in each pairwise comparison.}%
%     \label{fig:thresholdAllwError}%
% \end{figure}

% Second, for a fixed number of samples, we use the RASVthreshold and vary the threshold to understand the role the threshold has. We generate $U$ and $w$ as we did in the first set of experiments again with $d = 10$ and $n = 200$. Then for $t \in \{.05*i: i \in [20]\}$, we sample 10,000 pairs of pairwise comparisons and fit the MLE $\hat{w}$. This procedure is repeated 5 times. 

% Figure \ref{fig:thresholdSweep} shows the estimation error of $w^*$ over each choice of threshold and the Kendall tau correlation from the true ranking to the estimated ranking. The error bars is the standard deviation over the 5 trials. As expected, as the threshold increases, the salient feature preference model and the BTL with features model converge to the same model.
% % 

% \begin{figure}%
%     \centering
%     \subfloat{{\includegraphics[width=9cm]{synthetic_experiment_figs/w_error_threshold_sweep.pdf} }}%
%     \qquad
%     \subfloat{{\includegraphics[width=9cm]{synthetic_experiment_figs/kt_threshold_sweep.pdf} }}%
%     \caption{The affect of threshold when using RASVthreshold.}%
%     \label{fig:thresholdSweep}%
% \end{figure}

% What makes the salient feature preference model fundamentally different from the BTL model is that the salient feature preference model allows pairwise comparisons that disagree with the underlying true ranking, i.e., the salient feature preference model can model a pair of items for which $\langle U_{i}^{\tau_{t}(\{i,j\})} - U_{j}^{\tau_{t}(\{i,j\})}, w^* \rangle >0$ meaning item $i$ beats item $j$ with probability greater than 50\% when only compared to themselves yet $\langle U_{i} - U_{j}, w^* \rangle \leq 0$ meaning item $i$ is lower in the ranking than item $j$ when incorporating all features into the ranking judgment. See Figure \ref{fig:inconsistenciesThresholdSweep} that shows what percentage of pairwise comparisons over all pairwise comparisons disagree with the underlying true ranking for each choice of threshold. Similarly, the preference model can result in intransitives. One way to measure intransitivity in ranking data is to consider triplets of items $(i,j,k)$ \cite{cattelan2012models}. A triplet satisfies strong stochastic transitivity if $P_{ij} > .5$ and $P_{jk}>.5$ implies $P_{ik}> \max\{P_{ij}, P_{jk} \}$. A triplet satisfies moderate stochastic transitivity if if $P_{ij} > .5$ and $P_{jk}>.5$ implies $P_{ik}> \min\{P_{ij}, P_{jk} \}$. And finally a triplet satisfies weak stochastic transitivity if if $P_{ij} > .5$ and $P_{jk}>.5$ implies $P_{ik}> .5$. Out of all possible triplets, we record how many satisfies $P_{ij} > .5$ and $P_{jk}>.5$ and call this the number of valid triplets. Figure \ref{fig:intransitivitiesThresholdSweep} shows how the ratio of the number of weak, moderate, strong and the number of valid triplets changes as the threshold changes.

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/st_threshold_sweep.pdf}
%     \caption{The affect of varying the threshold on intransitivity for the RASVthreshold.}%
%     \label{fig:intransitivitiesThresholdSweep}%
% \end{figure}

% We also plot the low noise violation rate which is the fraction of pairs for which the low noise condition does not hold. See Figure \ref{fig:LNThresholdSweep}. The low noise condition is a property of the underlying pairwise probabilities and is defined as the following: if for any pair of items $(i,j)$ $P_{ij} > .5$, then $\sum_{k} P_{ki} > \sum_{k} P_{kj}$. The low noise condition is a sufficient condition for the MLE of the BTL without features model to produce a ranking that minimizes the number of pairs that disagree with the underlying ranking \cite{rajkumar2016can}.

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/inconsistency_threshold_sweep.pdf}
%     \caption{The affect of varying the threshold on pairwise inconsistency rate for the RASVthreshold.}%
%     \label{fig:inconsistenciesThresholdSweep}%
% \end{figure}

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/LN_threshold_sweep.pdf}
%     \caption{The affect of varying the threshold on low noise for the RASVthreshold.}%
%     \label{fig:LNThresholdSweep}%
% \end{figure}

% Since the salient feature preference model only uses some features for each pairwise comparison, it is interesting to see how many features on average each pairwise comparison uses. See Figure \ref{fig:avgNumFeaturesAndSat}.

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/avg_h_threshold_sweep.pdf}
%     \caption{The affect of varying the threshold on how many features are used in a pairwise comparison for the RASVthreshold.}%
%     \label{fig:avgNumFeaturesAndSat}%
% \end{figure}

% In order to illustrate Theorem \ref{thm:sampleComplexity}, for the threshold set to $t = .1$ and $t = .8$, we plot the estimation error of $w^*$ along with the predicted theoretical bound in Figure \ref{fig:thresholdSampleComplexity}.

% \begin{figure}%
%     \centering
%     \subfloat{{\includegraphics[width=8cm]{synthetic_experiment_figs/w_error_2_additive_thresh.pdf} }}%
%     \qquad
%     \subfloat{{\includegraphics[width=8cm]{synthetic_experiment_figs/kt_2_additive_thresh.pdf} }}%
%     \caption{RASVthreshold function with threshold $t = .2$}%
%     \label{fig:thresholdSampleComplexity}%
% \end{figure}

% We repeat the above experiments for the relative independent sample variance threshold function. 

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/w_error_threshold_sweep_indp.pdf}
%     \label{fig:wErrorThresholdSweepIndp}%
%     \caption{The affect of the threshold on estimation error under the relative independent sample variance threshold.}
% \end{figure}

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/kt_threshold_sweep_indp.pdf}
%     \label{fig:ktErrorThresholdSweepIndp}%
%     \caption{The affect of the threshold on estimated ranking with the relative independent sample variance threshold.}
% \end{figure}

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/st_threshold_sweep_indp.pdf}
%     \caption{The affect of the threshold on transitivity properties with the relative independent sample variance threshold.}
%     \label{fig:stThresholdSweepIndp}%
% \end{figure}

% \begin{figure}%
%     \centering
% \includegraphics[width=8cm]{synthetic_experiment_figs/LN_threshold_sweep_indp.pdf}
%     \caption{The affect of the threshold on low noise violations with the relative independent sample variance threshold.}
%     \label{fig:LNThresholdSweepIndp}%
% \end{figure}

% \begin{figure}%
%     \centering
%     \includegraphics[width=8cm]{synthetic_experiment_figs/avg_h_threshold_sweep_indp.pdf}
%     \caption{The affect of the threshold on how many features are used on average in a pairwise comparison that does not use all features with the relative independent sample variance threshold.}
%     \label{fig:avgHThresholdSweepIndp}%
% \end{figure}

% \begin{figure}%
%     \centering
%     \subfloat{{\includegraphics[width=8cm]{synthetic_experiment_figs/w_error_2_indp_thresh.pdf} }}%
%     \qquad
%     \subfloat{{\includegraphics[width=8cm]{synthetic_experiment_figs/kt_2_indp_thresh.pdf} }}%
%     \caption{Relative independent sample variance threshold function with threshold $t = .2$}%
%     \label{fig:thresholdSampleComplexity}%
% \end{figure}


% Third we consider different models for $U$ that result in a marked difference between the salient feature preference model and the BTL with features model with respect to the learned ranking. We sample the columns of $U$ from a mixture of 3 Gaussians whose means are drawn from $\mathcal{N}(0, 2I)$ such that each Gaussian has equal chance of being drawn. We set $d = 10$ and $n=200$.
